Imputation for High-Dimensional Linear Regression

We study high-dimensional regression with missing entries in the covariates. A common strategy in practice is to \emph{impute} the missing entries with an appropriate substitute and then implement a standard statistical procedure acting as if the covariates were fully observed. Recent literature on this subject proposes instead to design a specific, often complicated or non-convex, algorithm tailored to the case of missing covariates. We investigate a simpler approach where we fill-in the missing entries with their conditional mean given the observed covariates. We show that this imputation scheme coupled with standard off-the-shelf procedures such as the LASSO and square-root LASSO retains the minimax estimation rate in the random-design setting where the covariates are i.i.d.\ sub-Gaussian. We further show that the square-root LASSO remains \emph{pivotal} in this setting. It is often the case that the conditional expectation cannot be computed exactly and must be approximated from data. We study two cases where the covariates either follow an autoregressive (AR) process, or are jointly Gaussian with sparse precision matrix. We propose tractable estimators for the conditional expectation and then perform linear regression via LASSO, and show similar estimation rates in both cases. We complement our theoretical results with simulations on synthetic and semi-synthetic examples, illustrating not only the sharpness of our bounds, but also the broader utility of this strategy beyond our theoretical assumptions.

==> AREstimate.tex <==
\subsection{Proof of Lemma ~\ref{lem:ARapprox}}
\label{sec:ARLemma}
We restate the Lemma for convenience:
\begin{customlemma}{3.1}
Define $\hat{\phi}$ as in ~\eqref{eq:ARParamApprox}.  Then, with probability at
    least 
    \[2\text{exp}\left\{-\frac{c}{16}u_2^2\right\} \vee
        2\text{exp}\left\{-\frac{c}{4}u_2\right\} +
        \text{exp}\left\{-\frac{9}{8}u_2^2\right\}\]
\begin{align*}
\left\lvert \hat{\phi} - \phi \right\rvert \leq \frac{u_2}{\sqrt{n(p-1)}}\left(\frac{4}{3}\alpha^{-2} +
\frac{2}{3}\alpha^{-1}\right)
\end{align*}
\end{customlemma}
\noindent \begin{proofof}{Lemma~\ref{lem:ARapprox}}
    Let us first examine the numerator: $\frac{1}{n(p-1)}
    \sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)}$.  We
    have:
    \begin{align*}
        &\pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{\alpha^2 \phi}{1 - \phi^2} \right\rvert \geq t\right\} \\
        &= \sum_{\bM}\pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{\alpha^2 \phi}{1 - \phi^2} \right\rvert \geq t \mathrel{\Bigg|}\bM\right\}\pr\left\{\bM\right\}
    \end{align*}
    Let $N_M \equiv \sum_{i,a}\bM_{ia} \bM_{i(a-1)}$ and notice that $\E
    \left\{\frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p}
    \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)}\mathrel{\Bigg|}\bM\right\} =
    \frac{N_M \phi}{n(p-1)(1 - \phi^2)}$. By an application of the triangle
    inequality, we see that:
    \begin{align*}
        &\pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{\alpha^2 \phi}{1 - \phi^2} \right\rvert \geq
        t\mathrel{\Bigg|}\bM\right\} \\
        &\leq \pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{N_M \phi}{n(p-1)(1 - \phi^2)} \right\rvert \geq
        t - \left\lvert\frac{\phi}{1-\phi^2} \left(\alpha^2 -
        \frac{N_M}{n(p-1)}\right)\right\rvert\mathrel{\Bigg|}\bM\right\} 
    \end{align*}
    Now, consider flattening $\bX$ into the vector $\underline{\bX}$ which has
    distribution $N\left(0, \underline{\bSig}\right)$, where we define:
    \[\underline{\bSig} \equiv 
    \begin{bmatrix}
        \bSig & 0 & \dots & 0 \\
        0 & \bSig & \dots & 0 \\
        \vdots & \vdots & \dots & \vdots \\
        0 & 0 & \dots & \bSig
    \end{bmatrix}\]
    This implies that:
    \[
        \frac{1}{n(p-1)}\sum_{i,a} \bX_{ia}\bX_{i(a-1)} \bM_{ia}\bM_{i(a-1)}
        \stackrel{d}{=} \frac{1}{n(p-1)} \left\langle \bg,
        \underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}\bg\right\rangle 
    \]
    where $\bg \sim N(0, \bI_{np})$, $\bA \in \mathbb{R}^{np \times np}$ and
    \[
        \underline{\bA} =
        \begin{bmatrix}
        \bA_1 & 0 & \dots & 0 \\
        0 & \bA_2 & \dots & 0 \\
        \vdots & \vdots & \dots & \vdots \\
        0 & 0 & \dots & \bA_n
    \end{bmatrix}
    \]
    and $\left(\bA_{i}\right)_{jk} = \mathbbm{1}\left\{j = k + 1, \quad
    \bM_{ij}\bM_{ik} = 1\right\}$.  We will make use of the following
    Hanson-Wright inequality (see ~\cite{vershynin2018high} Theorem 6.2.1):
    \begin{align*}\pr\left\{\frac{1}{n(p-1)}\left\lvert \left\langle\bg,
        \underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}\bg\right\rangle
        - \E \left\langle\bg,
        \underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}\bg\right\rangle
        \right\rvert \geq t\right\} &\leq
        2\text{exp}\left\{-c\min\left\{\frac{t^2}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}^2},
        \frac{t}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{op}}\right\}\right\}
        \\
        &\leq
        2\text{exp}\left\{-c\frac{t^2}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}^2}\right\}
        \vee \text{exp}\left\{-c
        \frac{t}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}}\right\}
    \end{align*}
    where the last inequality follows by noting that $\norm{A}_{op} \leq
    \norm{A}_F$.  
    Now, let $\mathcal{M}_{\epsilon}$ be the event that $\left\lvert \alpha^2 -
    \frac{N_M}{n(p-1)}\right\rvert \leq \epsilon$ and notice that on this event
    $t - \left\lvert\frac{\phi}{1-\phi^2} \left(\alpha^2 -
        \frac{N_M}{n(p-1)}\right)\right\rvert \geq t - \frac{2}{3}\epsilon$.
        Thus, by the Hanson-Wright inequality above, we have:
    \begin{align*}
        &\sum_{\bM}\pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{\alpha^2 \phi}{1 - \phi^2} \right\rvert \geq t
        \mathrel{\Bigg|}\bM\right\}\pr\left\{\bM\right\} \\
        &\leq 2\text{exp}\left\{-c\frac{n^2(p-1)^2\left(t - \frac{2}{3}\epsilon\right)^2}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}^2}\right\}
        \vee 
        \text{exp}\left\{-c
        \frac{n(p-1)\left(t -\frac{2}{3}\epsilon\right)}{\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}}\right\}
        + \pr\left\{\mathcal{M}_{\epsilon}^{C}\right\}
    \end{align*}
We now compute
    \[\norm{\underline{\bSig}^{\frac{1}{2}}\underline{\bA}\underline{\bSig}^{\frac{1}{2}}}_{F}^2
    =
    \sum_{i=1}^{n}\norm{\bSig^{\frac{1}{2}}\bA_i\bSig^{\frac{1}{2}}}_{F}^2 \leq
    n\norm{\bSig^{\frac{1}{2}}\bA\bSig^{\frac{1}{2}}}_{F}^2\]
    where $\left(\bA\right)_{jk} = \mathbbm{1}\left\{j = k + 1\right\}$.  Noting
    the covariance structure of $\bSig$, we compute:
    \begin{align*}
        n\norm{\bSig^{\frac{1}{2}}\bA\bSig^{\frac{1}{2}}}_{F}^2 &=
        n\text{Tr}\left(\bSig^{\frac{1}{2}}\bA^{T}\bSig^{\frac{1}{2}}\bSig^{\frac{1}{2}}\bA\bSig^{\frac{1}{2}}\right)
        = n\text{Tr}\left(\bA\bSig\bA^T\bSig\right)
    \end{align*}
    Computing this trace gives:
    \begin{align*}
     n\text{Tr}\left(\bA\bSig\bA^T\bSig\right) &=n\sum_{a=2}^{p-1}\frac{\phi^2}{(1 - \phi^2)^2} \left(2 + \frac{2 -
    \phi^{2(a-1)} - \phi^{2(p-a)}}{1 - \phi^2}\right) \leq 4n(p-1)
    \end{align*}
    where the inequality is by using the assumption $\phi \leq \frac{1}{2}$.
    Which gives us the upper bound on the probability:
    \[2\text{exp}\left\{-\frac{c}{4}n(p-1)\left(t -
    \frac{2}{3}\epsilon\right)^2\right\} \vee
    \text{exp}\left\{-\frac{c}{2}\sqrt{n(p-1)}\left(t -
    \frac{2}{3}\epsilon\right)\right\} + \pr\left\{\mathcal{M}_{\epsilon}^{C}\right\}\]
    We now tackle $\pr\left\{\mathcal{M}_{\epsilon}^{C}\right\} =
    \pr\left\{\left\lvert\frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p}\bM_{ia}\bM_{i(a-1)}
    - \alpha^2\right\rvert \geq \epsilon\right\}$.  Notice that by Hoeffding's
    inequality for bounded random varibles (e.g. Theorem 2.2.6 in
    ~\cite{vershynin2018high}), we have:
    \[\pr\left\{\left\lvert\frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p}\bM_{ia}\bM_{i(a-1)}
    - \alpha^2\right\rvert \geq \epsilon\right\} \leq
    \text{exp}\left\{-2\epsilon^2 n(p-1)\right\}\]
    Taking $\epsilon = \frac{3 u_1}{2\sqrt{n}{p-1}}$, we have
    $\pr\left\{\mathcal{M}_{\epsilon}^{C}\right\} \leq
    \text{exp}\left\{-\frac{9}{2}u_1^2\right\}$.  Thus, taking $t =
    \frac{u_2}{\sqrt{n(p-1)}}$, we have:
    \begin{align*}
        &\pr\left\{\left\lvert \frac{1}{n(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{p} \bX_{ia}\bX_{i(a-1)}\bM_{ia} \bM_{i(a-1)} -
        \frac{\alpha^2 \phi}{1 - \phi^2} \right\rvert \geq \frac{u_2 -
        u_1}{\sqrt{n(p-1)}}\right\} \\
        &\leq 2\text{exp}\left\{-\frac{c}{4}\left(u_2 - u_1\right)^2\right\} \vee
        2\text{exp}\left\{-\frac{c}{2}\left(u_2 - u_1\right)\right\} + \text{exp}\left\{-\frac{9}{2}u_1^2\right\}
    \end{align*}
    We now tackle the denominator $\frac{1}{ n
(d-1)}\sum_{i=1}^{n}\sum_{a=2}^{d}\bX_{ia}^2 \bM_{ia}$.  We are interested in:
\begin{align*}
    \pr\left\{\left\lvert \frac{1}{n
    (d-1)}\sum_{i=1}^{n}\sum_{a=2}^{d}\bX_{ia}^2 \bM_{ia} - \frac{\alpha}{1 -
    \phi^2}\right\rvert \geq t\right\}
\end{align*}
To this end, we define the matrix $\bA \in \mathbb{R}^{np \times np}$:
\[ \bA \equiv
\begin{bmatrix}
    \bSig^{\frac{1}{2}}\left(\sum_{a=2}^{p}\be_a \be_a^T
    \bM_{1a}\right)\bSig^{\frac{1}{2}} & 0 &\dots & 0 \\
    0 &  \bSig^{\frac{1}{2}}\left(\sum_{a=2}^{p}\be_a \be_a^T
    \bM_{2a}\right)\bSig^{\frac{1}{2}} & \dots & 0 \\
    \vdots & \vdots & \cdots & \vdots \\
    0 & 0 & \dots &  \bSig^{\frac{1}{2}}\left(\sum_{a=2}^{p}\be_a \be_a^T
    \bM_{na}\right)\bSig^{\frac{1}{2}}
\end{bmatrix}
\]
We thus see that we can write our estimator $\frac{1}{ n
(p-1)}\sum_{i=1}^{n}\sum_{a=2}^{d}\bX_{ia}^2 \bM_{ia} = \frac{1}{ n
(p-1)}\left\langle \bg, \bA \bg \right\rangle$. Where $\bg \sim N(0, \bI_{np})$.
We can calculate $\norm{\bA}_{F}^2 \leq n
\norm{\bSig^{\frac{1}{2}}\left(\sum_{a=1}^{p}\be_a \be_a^T
    \right)\bSig^{\frac{1}{2}}}_{F}^2 = np\left(\frac{1 - \phi^{2p}}{\left(1 -
    \phi^2\right)^3}\right) \leq 8np$.  Using the same proof technique as above,
    and taking $\epsilon = \frac{3u_1}{4\sqrt{n(p-1)}}$ and $t =
    \frac{u_2}{\sqrt{n(p-1)}}$, we obtain:
    \begin{align*}
    \pr\left\{\left\lvert \frac{1}{n
    (d-1)}\sum_{i=1}^{n}\sum_{a=2}^{d}\bX_{ia}^2 \bM_{ia} - \frac{\alpha}{1 -
    \phi^2}\right\rvert \geq t\right\} \leq 2\text{exp}\left\{-\frac{c}{4}\left(u_2 - u_1\right)^2\right\} \vee
        2\text{exp}\left\{-\frac{c}{2}\left(u_2 - u_1\right)\right\} + \text{exp}\left\{-\frac{9}{2}u_1^2\right\} 
\end{align*}
and thus, we have $\left\lvert \hat{\phi} - \phi \right \rvert \leq
\frac{u_2}{\sqrt{n(p-1)}}\left(\frac{4}{3}\alpha^{-2} +
\frac{2}{3}\alpha^{-1}\right)$ and the probability guarantee comes by taking
$u_1 = \frac{1}{2}u_2$.
\end{proofof}


==> GeneratingFunctionBoundary.tex <==
\subsection{Moments of Markov Blankets}
\label{sec:BlanketSize}
\begin{customlemma}{5.1}
    \begin{itemize}
        \item[(i.)] $\E\left\{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
            \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2\right\} \leq
            \norm{\bbe_0}_1^2 \norm{\bSig}_{op} \E S_{(i,b)}^3$
    \item[(ii.)] $\E\left\{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
            \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^4\right\} \leq
            3\norm{\bbe_0}_1^4 \norm{\bSig}_{op}^2 \E S_{(i,b)}^6$
    \end{itemize}
    \end{customlemma}
\noindent\begin{proofof}{Lemma ~\ref{lem:ChebyshevControl}}
    \begin{itemize}
    \item[(i.)] We first expand:
        \begin{align*}
        \E\left\{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
            \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2\right\} =
            \E\left\{\sum_{b, c \in [p] \times [p]} \prod_{I \in \{b, c\}} \left\lvert\bbe_{0,I}\right\rvert\sqrt{S_{(i,I)}}\sum_{j
            \in S_{(i,I)}}\left\lvert\bX_{ij}\right\rvert\right\}
        \end{align*}
        We first look at the terms $b = c$ and the quantity of interest is thus
            $\E\left\{S_{(i,b)} \left(\sum_{j \in S_{(i,b)}}
            |\bX_{ij}|\right)^2\right\}$.  Noticing that $\E \bX_{ij}^2 \leq
            \norm{\bSig}_{op}$ and $\E \bX_{ij}\bX_{ik} \leq \norm{\bSig}_{op}$
            shows $\E\left\{S_{(i,b)} \left(\sum_{j \in S_{(i,b)}}
            |\bX_{ij}|\right)^2\right\} \leq \norm{\bSig}_{op} \E S_{(i,b)}^3$.
            Similarly noting that by Cauchy-Schwarz, $\E \sqrt{S_{(i,b)}
            S_{(i,c)}} \leq \E S_{i,b}$, we see that:
            \begin{align*}
            \E\left\{\sum_{b \neq c \in [p] \times [p]} \prod_{I \in \{b, c\}} \left\lvert\bbe_{0,I}\right\rvert\sqrt{S_{(i,I)}}\sum_{j
                \in S_{(i,I)}}\left\lvert\bX_{ij}\right\rvert\right\} &= \sum_{b
                \neq c \in [p] \times [p]} \prod_{I \in \{b, c\}} \left\lvert\bbe_{0,I}\right\rvert \E \left\{\sqrt{S_{(i,I)}}\sum_{j
                \in S_{(i,I)}}\left\lvert\bX_{ij}\right\rvert\right\} \\
                &\leq \sum_{b
                \neq c \in [p] \times [p]} \prod_{I \in \{b, c\}}
                \left\lvert\bbe_{0,I}\right\rvert \norm{\bSig}_{op} \E
                S_{(i,b)}^3
            \end{align*}
            Summing the two pieces gives the desired result.
        \item[(ii.)]  First notice that $4$ identically distributed, positive
            random variables $Y_1, Y_2, Y_3, Y_4$ are such that $\E Y_1 Y_2 Y_3 Y_4
            \leq E Y_1^4$.  One can see this by noticing that $Y_1 Y_2 Y_3 Y_4 \leq
            \frac{1}{2}\left((Y_1 Y_2)^2 + (Y_3Y_4)^2\right)$ and that $\E
            (Y_1Y_2)^2 \leq \E Y_1^4$ where the second inequality is by
            Cauchy-Schwarz.  Now, expanding and noting that $\E |\bX_{ij}|^4
            \leq 3 \norm{\bSig}_{op}^2$ gives the result (following the same
            recipe as above).
    \end{itemize}
\end{proofof}

In this section, we first control the $k$th moments of the Markov blanket and
then bound its moment generating function.  The overall techniques for both
lemmas are similar and involve upper bounding the quantity of interest by one on
a tree and performing a recursive computation.  We begin by stating and proving a lemma on the $k$th moments of the blanket.
\begin{lemma}
\label{lem:BlanketMoments}
    Suppose that $(1 - \alpha)(d_{\max} - 1)^k < 1$.  Then, for any node
    $S_{(i,b)}$:
    \begin{align*}
    \E S_{(i,b)}^k \leq \alpha + (1 - \alpha) d_{\max}^k \cdot \frac{\alpha}{1 -
        (1 - \alpha)(d_{\max} - 1)^k}
    \end{align*}
\end{lemma}
\noindent\begin{proofof}{Lemma ~\ref{lem:BlanketMoments}}
    Denote the graphical model by $G$.  Consider node $b$ and remove all cycles in
    the graph $G$ to create the new graph $T_{G}$.  Augment this tree to create
    the infinite rooted tree $T_{\infty}$ with degree $d_{\text{max}}$ and notice that the
    size of the boundary $\partial B_{T_{\infty}}(b)$ under the process where
    each node of the tree is marked with probability $\alpha$ is strictly larger than
    $S(i,b)$.  We thus work on the easier to control graph $T_{\infty}$.  Let
    $S_{\downarrow}$ denote the size of the Markov blanket of an intermediate
    looking down in the tree.  We then have the following recursions:
    \begin{align*}
        \E\left\{S^k \right\} &= \alpha + (1 - \alpha)
        \E\left\{\left(\sum_{i=1}^{d_{\max}}S_{\downarrow, i}\right)^k\right\}
        \\
        \E\left\{S_{\downarrow}^k \right\} &= \alpha + (1 - \alpha)
        \E\left\{\left(\sum_{i=1}^{d_{\max} - 1}S_{\downarrow, i}\right)^k\right\} 
    \end{align*}
    where $S_{\downarrow, i}$ are i.i.d. copies of $S_{\downarrow}$ (since the
    process is on an infinite tree).  Now, noting that $S_{\downarrow}$ are
    non-negative, we have by Jensen's inequality:
    \begin{align*}
        \left(\sum_{i=1}^{d_{\max} - 1}S_{\downarrow, i}\right)^k \leq
        (d_{\max} - 1)^{k - 1}\sum_{i=1}^{d_{\max} - 1} S_{\downarrow, i}^k
    \end{align*}
    The previous inequality and the condition $(1 - \alpha)(d_{\max} - 1)^k < 1$
    thus imply $\E\left\{S_{\downarrow}^k \right\} \leq \frac{\alpha}{1 - (1 -
    \alpha)(d_{\max} - 1)^k}$ by using the second recursion.  Plugging this
    inequality into the first recursion yields the desired result.
\end{proofof}

\noindent We now state and prove Lemma ~\ref{lem:generatingFunctionBoundary}
\begin{customlemma}{3.3}
    The random variables $S_{(i,b)}$ have sub-exponential tails.  That is, there
    exists a constant $C_{B}(\alpha, d_{\text{max}})$ depending only on $\alpha,
    d_{\text{max}}$ such that:
    \begin{align*}
        \pr\left\{S(i,b) \geq t\right\} \leq 2e^{-C_{B}(\alpha, d_{\text{max}})t}
    \end{align*}
\end{customlemma}
\noindent\begin{proofof}{Lemma ~\ref{lem:generatingFunctionBoundary}}
We again consider the upper bound on the tree and upper bound the size via tree
    recursions:
    \begin{align*}
        \E\left\{e^{\lambda S}\right\} &= \alpha e^{\lambda} +
        (1 - \alpha)\E\left\{e^{\lambda
        S_{\downarrow}}\right\}^{d_{\text{max}}} \\
        \E\left\{e^{\lambda S_{\downarrow}}\right\} &= \alpha e^{\lambda} +
        (1 - \alpha)\E\left\{e^{\lambda
        S_{\downarrow}}\right\}^{d_{\text{max}} - 1} 
    \end{align*}
    Let $\phi(\lambda) \equiv \E\left\{e^{\lambda
        S_{\downarrow}}\right\}$ and notice that $\phi(0) = 1$.
\end{proofof}


==> ProofsAR.tex <==
\subsection{Proof of Theorem ~\ref{thm:ARres}}
\begin{proofof}{Theorem ~\ref{thm:ARres}}
Throughout the proof we will use $\hat{\bX}$ to denote the exact conditional
expectation-imputed matrix and $\tilde{\bX}$ to denote the matrix whose
entries are imputed using the estimated value of $\hat{\phi}$.  The proof relies
on showing that the deviations $\hat{\bX} - \tilde{\bX}$ are not too large in
an appropriate sense.  To this end, we will show that taking $\lambda = \sigma_X^2\left(\sigma^2 +
        C\left(\sqrt{1 -
        \alpha}\right)R\right)\sqrt{\frac{\log{p}}{n}}$ allows us to bound each
        of the assumed terms in Lemma ~\ref{prop:GeneralLasso}.  Our general
        strategy for showing each of these assumptions will be to re-write
        $\tilde{\bX} = \left(\tilde{\bX} - \hat{\bX}\right) + \hat{\bX}$.
        We will then have a sequence of natural error terms (analogous for each term in
        the assumption) to analyze. 
We are first interested in showing
$\norm{\frac{1}{n}\tilde{\bX}^{T}\left(\tilde{\bX} - \bX\right)\bbe_0}_{\infty} \leq
\frac{\lambda}{4}$.  We re-write this and use the triangle inequality to see:
\begin{align*}
\norm{\frac{1}{n}\tilde{\bX}^{T}\left(\tilde{\bX} -
\bX\right)\bbe_0}_{\infty} &\leq  
\underbrace{\norm{\frac{1}{n}\hat{\bX}^T\left(\tilde{\bX} -
\hat{\bX}\right)\bbe_0}_{\infty}}_{A.} + \underbrace{\norm{\frac{1}{n}\left(\tilde{\bX} -
\hat{\bX}\right)^T\left(\tilde{\bX} - \hat{\bX}\right)\bbe_0}_{\infty}}_{B.}\\
&+ \underbrace{\norm{\frac{1}{n}\left(\tilde{\bX} -
\hat{\bX}\right)^T\left(\hat{\bX} - \bX\right)\bbe_0}_{\infty}}_{C.} 
 + 
\underbrace{\norm{\frac{1}{n}\hat{\bX}^T\left(\hat{\bX} - \bX\right)\bbe_0}_{\infty}}_{D.}
\end{align*}
We tackle each of these terms separately (noting that term D. was analyzed in
Theorem ~\ref{thm:mainres}).
\begin{enumerate}[align=left]
\item[A.] We re-write this term as $\max_{a \in [p]}\left\lvert\frac{1}{n}
\sum_{i=1}^{n}\sum_{b=1}^{d}\hat{\bX}_{ia}\left(\tilde{\bX}_{ib}
-\hat{\bX}_{ib}\right)\bbe_{0,b}\right\rvert$.  Let $S_i \subseteq [p]$ denote the
(random) set which consists of the indices of the variables observed in row $i$.
Then, for some entry in the row $\E\left\{\bX_{ik} \mid \bX_{S_i}\right\} =
\E\left\{\bX_{ik} \mid \bX_{i, L(k)}, \bX_{i, R(k)}\right\}$ where $L(k)$ is the
random variable denoting the index of the closest observed entry to the left of
$k$ and $R(k)$ is the analogous quantity on the right (see Figure
~\ref{fig:graph_mod_AR1}).  
%\input{figs/graphicalModel.tex}

Thus since each row is a multivariate Gaussian, we
can write the following two quantities:
\begin{align*}
&\hat{\bX}_{ik} = \frac{\phi^{d_1 + d_2}}{1 - \phi^{2(d_1 + d_2)}}
    \left(\bX_{i,L(k)}\left(\phi^{-d_2} - \phi^{d_2}\right) + \bX_{i, R(k)} \left(\phi^{-d_1} -
    \phi^{d_1}\right)\right) \\
&\tilde{\bX}_{ik} = \frac{\hat{\phi}^{d_1 + d_2}}{1 - \hat{\phi}^{2(d_1 + d_2)}}
    \left(\bX_{i, L(k)}\left(\hat{\phi}^{-d_2} - \hat{\phi}^{d_2}\right) +
    \bX_{i, R(k)} \left(\hat{\phi}^{-d_1} -
    \hat{\phi}^{d_1}\right)\right)
\end{align*}
where we have used $d_1 \equiv k - L(k)$, $d_2 \equiv R(k) - k$. We again write
this more succinctly, letting $f_L(\phi) = \frac{\phi^{d_1 + d_2}}{1 - \phi^{2(d_1 + d_2)}}
    \left(\phi^{-d_2} - \phi^{d_2}\right)$ and $f_R(\phi) = \frac{\phi^{d_1 + d_2}}{1 - \phi^{2(d_1 + d_2)}}
    \left(\phi^{-d_1} - \phi^{d_1}\right)$.  
We can thus re-write $\tilde{\bX}_{ik} -
\hat{\bX}_{ik} = \left(\hat{\phi} - \phi\right)\left(\bX_{i, L(k)}f_L^{'}(\xi_L)
+ \bX_{i, R(k)}f_R^{'}(\xi_R)\right)$ for some $\xi_L, \xi_R \in \left(\phi,
\hat{\phi}\right)$ by the mean-value theorem.  Thus, we have:
\begin{align*}
\max_{a \in [p]}\left\lvert\frac{1}{n}
\sum_{i, b}\hat{\bX}_{ia}\left(\tilde{\bX}_{ib}
-\hat{\bX}_{ib}\right)\bbe_{0,b}\right\rvert &= \max_{a \in [p]}\Biggl\lvert
\frac{1}{n}\sum_{i,b}\hat{\bX}_{ia}\left(\hat{\phi} -
\phi\right) \left(\bX_{i, L(b)}f_L^{'}(\xi_{L}) + \bX_{i,
R}f_R^{'}(\xi_{R})\right)\bbe_{0,b}\Biggr\rvert \\
&\leq \left\lvert
\hat{\phi} - \phi \right\rvert\max_{a \in [p]} \sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert
\frac{1}{n}\sum_{i=1}^{n}\left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
    L(b)}\right\rvert \left\lvert f_L^{'}(\xi_{L(b)})\right\rvert \\
&+ \left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
    R(b)}\right\rvert \left\lvert f_R^{'}(\xi_{R(b)})\right\rvert  \\
    &\stackrel{(a.)}{\leq} \frac{u_2 C(\alpha)}{\sqrt{np}}
\max_{a}\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\frac{1}{n}\sum_{i=1}^{n}\left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
L(b)}\right\rvert + \left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
R(b)}\right\rvert 
\end{align*}
where (a.) holds on the event $\mathcal{A}_1$, the event on which the result of
Lemma ~\ref{lem:ARapprox} holds and since the derivatives are uniformly bounded
by a universal constant $C$.  Notice that we are now able to use
independence across the coordinates $i$ as we have pulled out the nuisance term
$\left\lvert \hat{\phi} - \phi \right\rvert$.  Notice now that $\hat{\bX}_{ia},
\bX_{i, L(b)}, \hat{\bX}_{ia}, \bX_{i, R(b)}$ are each sub-Gaussian with
parameter $\sigma_X^2$.  Thus, notice that each of the variables $\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert$ and $\left\lvert
        \hat{\bX}_{ia}\bX_{i, R(b)} \right \rvert$ are sub-Exponential (by
        Lemma~\ref{lem:productsubGaussian}).  Now, fixing a pair $a,b$, and
        taking $t < 16e\sigma_X^2$, we can see
that:
\begin{align*}
\pr\left\{\left\lvert\frac{1}{n}\sum_{i=1}^{n}\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert - \E\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert \right\rvert \geq t\right\} \leq
2\text{exp}\left\{-\frac{nt^2}{256e^2\sigma_X^4}\right\}
\end{align*}
Taking $t = 16eA\sigma_X^2\sqrt{\frac{\log{p}}{n}}$, we see that:
\begin{align*}
\pr\left\{\max_{a,b \in [p] \times [p]}\left\lvert\frac{1}{n}\sum_{i=1}^{n}\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert - \E\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert \right\rvert \geq t\right\} \leq p^{2
    - A^2}
\end{align*}
Letting $\mathcal{A}_2$ denote the event on which the above does not hold and noting
that $E\left\lvert
\hat{\bX}_{ia}\bX_{i, L(b)} \right \rvert$ is a constant, we see that on
$\mathcal{A}_1 \cap \mathcal{A}_2$:
\begin{align*}
    \frac{C(\alpha)u_2}{\sqrt{np}}
\max_{a}\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\frac{1}{n}\sum_{i=1}^{n}\left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
L(b)}\right\rvert + \left\lvert\hat{\bX}_{ia}\right\rvert\left\lvert\bX_{i,
    R(b)}\right\rvert \leq \frac{C(\alpha)u_2}{\sqrt{np}}\norm{\bbe_0}_1 
\end{align*}
Finally, this last quantity can be upper bounded by $C(\alpha)R\sqrt{\frac{\log{p}}{n}}$
using Cauchy-Schwarz, taking $u_2 =\sqrt{\log{p}}$, and the fact that $s < p$. 
\item[B.] The technique is essentially identical to term A.  We write:
\begin{align*}
\norm{\frac{1}{n}\left(\tilde{\bX} -
\hat{\bX}\right)^T\left(\tilde{\bX} - \hat{\bX}\right)\bbe_0}_{\infty} &=
\max_{a \in [p]}\Biggl\lvert
\frac{1}{n}\sum_{i,b}\left(\hat{\phi} -
\phi\right)^2 \prod_{k \in \{a, b\}}\left(\bX_{i, L(k)}f_L^{'}(\xi_{L}) + \bX_{i,
R(k)}f_R^{'}(\xi_{R})\right)\bbe_{0,b}\Biggr\rvert \\
    &\leq \frac{C(\alpha)u_2^2}{np}\norm{\bbe_0}_1
\end{align*}
on $\mathcal{A}_1 \cap \mathcal{A}_2$.  As before this quantity can
be upper bounded by $C(\alpha)R\sqrt{\frac{\log{p}}{n}}$ using the same techniques.
\item[C.] The proof of this upper bound is identical to term A.
\end{enumerate}

We now must tackle the term $\norm{\frac{1}{n}\tilde{\bX}^T\beps}_{\infty}$.  As
before, we have:
\begin{align*}
\norm{\frac{1}{n}\tilde{\bX}^T\beps}_{\infty} &\leq \norm{\frac{1}{n}\left(\tilde{\bX}
- \hat{\bX}\right)^T\beps}_{\infty} +
\norm{\frac{1}{n}\hat{\bX}^T\beps}_{\infty} \\
&= \left\lvert \sum_{i=1}^{n}\frac{1}{n}\left(\hat{\phi} -
\phi\right)\left(\bX_{i, L(a)}f_{L}^{'}(\xi_L) - \bX_{i,
R(a)}f_{R}^{'}(\xi_R)\right)\beps_i\right\rvert  +
\norm{\frac{1}{n}\hat{\bX}^T\beps}_{\infty} \\
    &\leq C(\alpha)\sigma \sigma_X\sqrt{\frac{\log{p}}{n}}
\end{align*}
where the last line holds with high probability using the same technique as term
A.  

Finally, we must analyze the quantity: 
$\sup_{\bw \in \mathcal{C} \cap
S^{p-1}}\frac{1}{n}\norm{\tilde{\bX} \bw}_2^2$
Using the same decomposition as above, we notice that:
\begin{align*}
\sup_{\bw \in \mathcal{C} \cap S^{p-1}}\frac{1}{n}\norm{\bX \bw}_2^2 &\geq
\sup_{\bw \in \mathcal{C} \cap S^{p-1}} \frac{1}{n}\norm{\hat{\bX}\bw}_2^2 -
\Biggl\lvert
\Biggl\langle\bw, \Biggl(\left(\tilde{\bX} - \hat{\bX}\right)^T\left(\tilde{\bX} -
\hat{\bX}\right) + \\
&\left(\tilde{\bX} - \hat{\bX}\right)^T\hat{\bX} +
\hat{\bX}^T\left(\tilde{\bX} - \hat{\bX}\right)\Biggr)\bw\Biggr\rangle
\Biggr\rvert \\
&\geq \sup_{\bw \in \mathcal{C} \cap S^{p-1}} \frac{1}{n}\norm{\hat{\bX}\bw}_2^2
- \norm{\bw}_1\Biggl(\norm{\left(\tilde{\bX} - \hat{\bX}\right)^T\left(\tilde{\bX} -
\hat{\bX}\right)\bw}_{\infty} \\
&+ \norm{\left(\tilde{\bX} -
\hat{\bX}\right)^T\hat{\bX}\bw}_{\infty} + \norm{\hat{\bX}^T\left(\tilde{\bX} -
\hat{\bX}\right)\bw}_{\infty} \Biggr) \\
&\geq \frac{\lambda_{\text{min}}\left(\Sigma_{\hat{\bX}}\right)}{4} 
\end{align*}
where the last inequality holds with high probability by the same proof as terms
$A, B, C$, the assumption on $s, p, n$ and Lemma ~\ref{lem:RE_Condition}.
\end{proofof}


==> ProofsBoundedDegreeGaussian.tex <==
\subsection{Proof of Theorem ~\ref{thm:GaussianRes}}
\label{subsec:proofsbounded}
\noindent \begin{proofof}{Theorem ~\ref{thm:GaussianRes}}
The proof largely follows the same program as Theorem ~\ref{thm:ARres}.  To this
end, we first examine:
\begin{align*}
\norm{\frac{1}{n}\widetilde{\bX}^{T}\left(\widetilde{\bX} -
\bX\right)\bbe_0}_{\infty} &\leq  
\underbrace{\norm{\frac{1}{n}\widehat{\bX}^T\left(\widetilde{\bX} -
\widehat{\bX}\right)\bbe_0}_{\infty}}_{A.} + \underbrace{\norm{\frac{1}{n}\left(\widetilde{\bX} -
\widehat{\bX}\right)^T\left(\widetilde{\bX} - \widehat{\bX}\right)\bbe_0}_{\infty}}_{B.}\\
&+ \underbrace{\norm{\frac{1}{n}\left(\widetilde{\bX} -
\widehat{\bX}\right)^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty}}_{C.} 
 + 
\underbrace{\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty}}_{D.}
\end{align*}
Unlike the previous example, controlling term A. does not give control over all
the terms.  Nonetheless, we begin by analyzing term A.
We write:
\begin{align*}
\norm{\frac{1}{n}\widehat{\bX}^T\left(\widetilde{\bX} -
\widehat{\bX}\right)\bbe_0}_{\infty} &= \max_{a = 1, 2, \dots, p}\left\lvert\frac{1}{n}
    \sum_{i=1}^{n}\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
-\widehat{\bX}_{ib}\right)\bbe_{0,b}\right\rvert\\
    &\leq \max_{a \in
    1, 2, \dots,
    p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left\lvert\widehat{\bX}_{ia}\right\rvert^2}
    \cdot \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
    -\widehat{\bX}_{ib}\right)\bbe_{0,b}\right)^2} 
\end{align*}
where the inequality is by Cauchy-Schwarz over the indices $i$. Our strategy is
then to upper bound each of the square root terms separately.  The more
    difficult term is the second, so we begin there, first by re-writing the
    approximate conditional expectation explicitly:
    \begin{align*}
    \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
        -\widehat{\bX}_{ib}\right)\bbe_{0,b}\right)^2} &= \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\left(\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}\right)\bX_{S(i,b)}\right\rvert\right)^2} 
    \end{align*}
    An application of H{\"o}lder's inequality (noting that $\left(\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}\right)$ is a row vector) yields the following upper bound:
    \begin{equation}
    \label{eq:TermAUpperBound}
\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\norm{\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2}
    \end{equation}
The key difficulty is that each of the terms is correlated across indices $i$ in
    a complicated manner,
    so we are unable to immediately use standard concentration inequalities on
    the sum.  To deal with this, we will uniformly upper-bound each of these
    terms which correlate the terms in the sum.
To this end, we have:
    \begin{align*}
\norm{\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty} &\leq \norm{\left(\bSig_{b, S_{(i,b)}} -
        \widetilde{\bSig}_{b, S_{(i,b)}}\right)\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty} + \\
        &\norm{\widetilde{\bSig}_{b, S_{(i,b)}}\left(\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}\right)}_{\infty}
    \end{align*}
We examine the second term first.  Note that for some vector $\bx \in
\mathbb{R}^{d}$ and square matrix $\bA \in \mathbb{R}^{d \times d}$, we have the
following inequality (letting $\bA^{(i)}$ denote the $i$th column of $\bA$):
\begin{align*}
    \norm{\bx^T \bA}_{\infty} = \max_{i = 1, 2, \dots, d}\left\lvert\left\langle
    \bx, \bA^{(i)}\right\rangle\right\rvert \leq \max_{i=1,2,\dots, d}
    \norm{\bx}_{\infty} \norm{\bA^{(i)}}_{1} \leq \sqrt{d}\max_{i = 1, \dots, d}
    \norm{\bx}_{\infty} \norm{\bA^{(i)}}_{2} \leq
    \sqrt{d}\norm{\bx}_{\infty}\norm{\bA}_{op}
\end{align*}
which implies immediately:
    \begin{align*}
\norm{\widetilde{\bSig}_{b, S_{(i,b)}}\left(\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}\right)}_{\infty} &\leq \norm{\widetilde{\bSig}_{b,
        S_{(i,b)}}}_{\infty}\sqrt{S_{(i,b)}}\norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op}
\end{align*}
Our strategy will be to take the power series
    expansion of $\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1} = \left(\bSig_{S_{(i,b)},
        S_{(i,b)}} + \bW_{S_{(i,b)},
        S_{(i,b)}}\right)^{-1}$, where for convenience we have used $\bW_{S_{(i,b)},
        S_{(i,b)}} = \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}} - \bSig_{S_{(i,b)},
        S_{(i,b)}}$.  Recall that by Lemma ~\ref{lem:operatorMissing} i., with
        probability at least $1 - e^{-u}$, $\norm{\widetilde{\bSig}_{SS} - \bSig_{SS}}_{op} \leq
            \frac{64e(1-\alpha)\norm{\bSig}_{op}}{\alpha^2}\sqrt{\frac{|S| +
            u}{n}}$ as long as $\sqrt{\frac{|S| + u}{n}} \leq \frac{1}{2}$.  Let
            $\mathcal{A}_O = \left\{\norm{\bW_{S_{(i,b)},
        S_{(i,b)}}}_{op} \leq
            \frac{64e(1-\alpha)\norm{\bSig}_{op}}{\alpha^2}\sqrt{\frac{|S_{(i,b)}| +
            2\log{2np}}{n}} \right\}$.  We will additionally need control on
            $|S(i,b)|$.
Let event $\mathcal{A}_B$ denote the event that the size of the Markov blankets
behave ``nicely", i.e. $\mathcal{A}_B = \left\{|S(i,b)| \leq
\frac{2}{C_B(\alpha, d_{\max})}\log{2np} \quad \forall i \in [n], b \in
[p]\right\}$ and notice that Lemma ~\ref{lem:generatingFunctionBoundary} implies
$\pr\left\{\mathcal{A}_B\right\} \geq 1 - \frac{1}{2np}$.  Now, on the event
$\mathcal{A}_O \cap \mathcal{A}_B$, we have:
\begin{align*}
\norm{\bW_{S_{(i,b)},
        S_{(i,b)}}}_{op} \leq
            \frac{64e(1-\alpha)\norm{\bSig}_{op}\left(1 + \frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2}\sqrt{\frac{\log{2np}}{n}}
\end{align*}
Noticing that by assumption $\frac{64e(1-\alpha)\norm{\bSig}_{op}\left(1 +
\frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2}\sqrt{\frac{\log{2np}}{n}} <
1$, so we can take the power series expansion of $\left(\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}} - \bSig_{S_{(i,b)},
        S_{(i,b)}}\right)^{-1}$ and we see thus that:
        \begin{align*}
        \norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op} 
        &\leq \norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op}\sum_{k=1}^{\infty}\norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op}^{k}\norm{\bW_{S_{(i,b)},
        S_{(i,b)}}}_{op}^{k} \\
        &\leq
            \frac{128e(1-\alpha)\norm{\bSig}_{op}\left(1 +
\frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2
\lambda_{\text{min}}(\bSig)^2}\sqrt{\frac{\log{2np}}{n}}
    \end{align*}
    where in the first inequality we have used the power series expansion, the
    triangle inequality, and the sub-multiplicativity of the operator norm and
    the second inequality used the assumption that $\frac{64e(1-\alpha)\norm{\bSig}_{op}\left(1 +
\frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2
\lambda_{\text{min}}(\bSig)}\sqrt{\frac{\log{2np}}{n}} < \frac{1}{2}$. Now, let
$\mathcal{A}_M$ denote the event that $\norm{\widetilde{\bSig} - \bSig}_{\ell_1 \rightarrow
        \ell_{\infty}} \leq \frac{64
        e\norm{\bSig}_{op}}{\alpha^2}\sqrt{\frac{\log{p}}{n}}$.  Then on the
        event $\mathcal{A}_M \cap \mathcal{A}_O \cap \mathcal{A}_B$ and assuming
        that $\frac{64e}{\alpha^2}\sqrt{\frac{\log{p}}{n}} \leq 1$, we
    upper bound the overall term by:
    \begin{align*}
\norm{\widetilde{\bSig}_{b, S_{(i,b)}}\left(\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}\right)}_{\infty} &\leq \norm{\widetilde{\bSig}_{b,
        S_{(i,b)}}}_{\infty}\sqrt{S_{(i,b)}}\norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} - \widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op} \\
        &\leq \frac{128e(1-\alpha)\norm{\bSig}_{op}^{2}\left(1 +
\frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2
        \lambda_{\text{min}}(\bSig)^2}\sqrt{|S_{(i,b)}|}\sqrt{\frac{\log{2np}}{n}}
    \end{align*}
    Similarly, we see that (working on the same event):
    \begin{align*}
    \norm{\left(\bSig_{b, S_{(i,b)}} -
        \widetilde{\bSig}_{b, S_{(i,b)}}\right)\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty} &\leq \norm{\bSig_{b, S_{(i,b)}} -
        \widetilde{\bSig}_{b,
        S_{(i,b)}}}_{\infty}\sqrt{S(i,b)}\norm{\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{op} \\
        &\leq
        \frac{64e\norm{\bSig}_{op}}{\alpha^2\lambda_{\text{min}}(\bSig)}\sqrt{\frac{\log{p}}{n}}\sqrt{S_{(i,b)}}
    \end{align*}
    Thus, we see that $\norm{\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty}$ is upper bounded by:
    \begin{align*}
        \sqrt{|S_{(i,b)}|}
        \sqrt{\frac{\log{2np}}{n}}\underbrace{\left(\frac{128e(1-\alpha)\norm{\bSig}_{op}^{2}\left(1 +
\frac{2}{C_B(\alpha, d_{\max})}\right)}{\alpha^2
        \lambda_{\text{min}}(\bSig)^2} +
        \frac{64e\norm{\bSig}_{op}}{\alpha^2\lambda_{\text{min}}(\bSig)}\right)}_{C_A}
    \end{align*}
    We now return to Eq.
    ~\ref{eq:TermAUpperBound} and upper bound as follows:
    \begin{align*}
        &\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\norm{\bSig_{b, S_{(i,b)}}\bSig_{S_{(i,b)},
        S_{(i,b)}}^{-1} -  \widetilde{\bSig}_{b, S_{(i,b)}}\widetilde{\bSig}_{S_{(i,b)},
        S_{(i,b)}}^{-1}}_{\infty}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2} \\
        &\leq C_A \sqrt{\frac{\log{2np}}{n}} \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2}
    \end{align*}
    Now, we notice that the quantity $\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2$  should concentrate,
    but since maximum control is not necessary, it suffices to use a simpler
    inequality such as Chebyshev.  We then need some control on the moments of
    the random variable $\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert$ which is done in the
    following lemma whose proof is deferred to the appendix:
    \begin{lemma}
    \label{lem:ChebyshevControl}
    \begin{itemize}
        \item[(i.)] $\E\left\{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
            \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2\right\} \leq
            \norm{\bbe_0}_1^2 \norm{\bSig}_{op} \E S_{(i,b)}^3$
    \item[(ii.)] $\E\left\{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
            \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^4\right\} \leq
            3\norm{\bbe_0}_1^4 \norm{\bSig}_{op}^2 \E S_{(i,b)}^6$
    \end{itemize}
    \end{lemma}
    Now, let $\mathcal{A}_{C}$ denote the event that 
    \begin{align*}
        \frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
    \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2 \leq
    \norm{\bSig}_{op}R^2s \left(\E S_{(i,b)}^3 + \sqrt{3 \E
    S_{(i,b)}^6}\right)
    \end{align*}
    Now, using the following lemma on the moments of $S_{(i,b)}$ (whose proof is
    deferred to the appendix):
    \begin{lemma}
\label{lem:BlanketMoments}
    Suppose that $(1 - \alpha)(d_{\max} - 1)^k < 1$.  Then, for any node
    $S_{(i,b)}$:
    \begin{align*}
    \E S_{(i,b)}^k \leq \alpha + (1 - \alpha) d_{\max}^k \cdot \frac{\alpha}{1 -
        (1 - \alpha)(d_{\max} - 1)^k}
    \end{align*}
\end{lemma}
we conclude that on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap
\mathcal{A}_B \cap \mathcal{A}_C$, 
\begin{align*}
\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
        -\widehat{\bX}_{ib}\right)\bbe_{0,b}\right)^2} \leq  C_{B} R \sqrt{\frac{s
        \log{2np}}{n}}
\end{align*}
where $C_B = C_A \cdot \norm{\bSig}_{op}\left(\E S_{(i,b)}^3 + \sqrt{3 \E
    S_{(i,b)}^6}\right)$.
Finally, let $\mathcal{A}_S$ be the event that $\max_{a \in 1, 2, \dots, p}
\frac{1}{n}\sum_{i=1}^{n} \bX_{ia}^2 \leq
    \norm{\bSig}_{op} + 16e\norm{\bSig}_{op}\sqrt{\frac{\log{p}}{n}}$.  Note that
    $\E\bX_{1a}^2 \leq \norm{\bSig}_{op}$, so we have: 
   \begin{align*}
\pr\left\{\max_{a \in 1, 2, \dots, p} \frac{1}{n}\sum_{i=1}^{n} \bX_{ia}^2 \geq
       \E \norm{\bSig}_{op} + t\right\} \leq \pr\left\{\max_{a \in 1, 2, \dots, p} \frac{1}{n}\sum_{i=1}^{n} \bX_{ia}^2 \geq
    \E \bX_{1a}^2 + t\right\} \leq
    \text{exp}\left\{-\frac{nt^2}{128e^2\norm{\bSig}_{op}^2} + \log{p}\right\}
\end{align*} 
Where the last inequality follows by
Lemma ~\ref{lem:subGaussianSquared} and taking $t = 16e\norm{\bSig}_{op}\sqrt{\frac{\log{p}}{n}}$ (under assumption
$\sqrt{\frac{\log{p}}{n}} \leq \frac{1}{2}$) yields
$\pr\left\{\mathcal{A}_S\right\} \geq 1 - \frac{1}{p}$.  For simplicity, by the
assumption on $\sqrt{\frac{\log{p}}{n}}$, we will note that on the event
$\mathcal{A}_S$, $\max_{a \in 1, 2, \dots, p}
\frac{1}{n}\sum_{i=1}^{n} \bX_{ia}^2 \leq 9e\norm{\bSig}_{op}$.  Thus, on the
event $\mathcal{A}_M \cap \mathcal{A}_O \cap
\mathcal{A}_B \cap \mathcal{A}_C \cap \mathcal{A}_S$, we have:
\begin{align*}
    \norm{\frac{1}{n}\widehat{\bX}^T\left(\widetilde{\bX} -
        \widehat{\bX}\right)\bbe_0}_{\infty} \leq 9e\norm{\bSig}_{op} C_B R
        \sqrt{\frac{s \log{2np}}{n}} = c(\alpha, d_{\max}, \norm{\bSig}_{op},
        \lambda_{\min}(\bSig))R\sqrt{\frac{s \log{2np}}{n}}
\end{align*}
where $c(\alpha, d_{\max}, \norm{\bSig}_{op},
        \lambda_{\min}(\bSig))$ is a constant which is independent of the
        parameters $R, s, n, p$.  We are now ready to tackle term B.  As before,
        we will write:
        \begin{align*}
        \norm{\frac{1}{n}\left(\widetilde{\bX} -
            \widehat{\bX}\right)^T\left(\widetilde{\bX} -
            \widehat{\bX}\right)\bbe_0}_{\infty} &= \max_{a = 1, 2, \dots, p}\left\lvert\frac{1}{n}
            \sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
            \widehat{\bX}_{ia}\right)\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
-\widehat{\bX}_{ib}\right)\bbe_{0,b}\right\rvert\\
    &\leq \max_{a \in
    1, 2, \dots,
            p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} - \widehat{\bX}_{ia}\right)^2}
    \cdot \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sum_{b=1}^{p}\left(\widetilde{\bX}_{ib}
    -\widehat{\bX}_{ib}\right)\bbe_{0,b}\right)^2}
        \end{align*}
As before, we see that on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap
\mathcal{A}_B$:
    \begin{align*}
        \max_{a \in
    1, 2, \dots,
            p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
            \widehat{\bX}_{ia}\right)^2} &\leq \max_{a \in [p]}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\norm{\bSig_{a, S_{(i,a)}}\bSig_{S_{(i,a)},
        S_{(i,a)}}^{-1} -  \widetilde{\bSig}_{a, S_{(i,a)}}\widetilde{\bSig}_{S_{(i,a)},
        S_{(i,a)}}^{-1}}_{\infty}\sum_{j
    \in S_{(i,a)}}\left\lvert\bX_{ij}\right\rvert\right)^2}\\
        &\leq C_{A}\sqrt{\frac{\log{2np}}{n}}\max_{a \in
        [p]}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2}
    \end{align*}
    We proceed by obtaining tail bounds on the quantity $\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2$ and using this
        to find an exponential tail bound on the empirical average from which
        point we can conclude with a union bound.  Notice that
    \begin{align*}
        \pr\left\{S_{(i,a)}\sum_{\ell,j \in S_{(i,a)} \times S_{(i,a)}}\left\lvert
        \bX_{ij}\bX_{i\ell}\right\rvert \geq t\right\} &= \sum_{k =1}^{p}
        \pr\left\{\sum_{\ell,j \in S_{(i,a)} \times S_{(i,a)}}\left\lvert
        \bX_{ij}\bX_{i\ell}\right\rvert \geq
        \frac{t}{k}\right\} \pr\left\{S_{(i,a)} = k\right\} \\
        &\leq
        \sum_{k=1}^{\infty}4\text{exp}\left\{-\frac{t}{16e\norm{\bSig}_{op} k^3} -
        C_B(\alpha, d_{\text{max}})k\right\}
    \end{align*}
    Now, we balance terms in the infinite sum around $t^{\frac{1}{4}}$ to see:
    \begin{align*}
    \sum_{k=1}^{\infty}4\text{exp}\left\{-\frac{t}{16e\norm{\bSig}_{op} k^3} -
        C_B(\alpha, d_{\text{max}})k\right\} &\leq
        4e^{-at^{\frac{1}{4}}}\sum_{k=1}^{\infty}\text{exp}\left\{at^{\frac{1}{4}}
        - \frac{t + 16e\norm{\bSig}_{op} C_B(\alpha,
        d_{\max})k^4}{16e\norm{\bSig}_{op}k^3}\right\} \\
        &\leq 4e^{-at^{\frac{1}{4}}} \Biggl(\sum_{k \leq t^{1/4}}\text{exp}\left\{at^{\frac{1}{4}}
        - \frac{t + 16e\norm{\bSig}_{op} C_B(\alpha,
        d_{\max})k^4}{16e\norm{\bSig}_{op}k^3}\right\}\\
        & + \sum_{k > t^{1/4}}\text{exp}\left\{at^{\frac{1}{4}}
        - \frac{t + 16e\norm{\bSig}_{op} C_B(\alpha,
        d_{\max})k^4}{16e\norm{\bSig}_{op}k^3}\right\}\Biggr) \\
        &\leq \frac{4}{1 - e^{-C_B(\alpha, d_{\max})/2}}e^{-at^{\frac{1}{4}}}
    \end{align*}
    where we have taken $a$ such that $a < \frac{1}{16e\norm{\bSig}_{op}} \wedge
    \frac{C_B(\alpha, d_{\max})}{2}$. Now, assuming 
    \[t < \frac{128e}{a -  ae^{-C_B(\alpha, d_{\max})/2}}\left(n
    \frac{a -  ae^{-C_B(\alpha, d_{\max})/2}}{1024e^2}\right)^{3}\] 
    by Lemma~\ref{lem:truncation}, we have: 
    \begin{align*}
        &\pr\left\{\frac{1}{n}\sum_{i=1}^{n}\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2 \geq 2\left(t + \E \left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2\right)\right\}
        \\
        &\leq 2
        \text{exp}\left\{-a\left(n t^2\frac{a -  ae^{-C_B(\alpha, d_{\max})/2}}{1024e^2}\right)^{\frac{1}{7}}
        + \log{n\left(\frac{4}{1 - e^{-C_B(\alpha, d_{\max})/2}}\right)}\right\}
    \end{align*}
    Thus, let $\mathcal{A}_{T}$ be the event that 
    \[\max_{a \in 1, 2, \dots, p}\frac{1}{n}\sum_{i=1}^{n}\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2 \leq
        2\left(A\sqrt{\frac{(\log{c_1 np})^7}{n}} + \E \left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2\right) \]
    where $c_1 = 2 + \frac{4}{1 - e^{-C_B(\alpha, d_{\max})/2}}$ and note that
    $\pr\left\{\mathcal{A}_T\right\} \geq 1 - \text{exp}\left\{\left(1 - c_2
    A^{2/7}\right)\log{c_1 np}\right\}$ where $c_2 = a \left(\frac{a -
    ae^{-C_B(\alpha, d_{\max})/2}}{1024e^2}\right)^{1/7}$.  Thus, on the event
    $\mathcal{A}_T$, and assuming $A\sqrt{\frac{(\log{c_1 np})^7}{n}} \leq
    \norm{\bSig}_{op} \E S_{(i,a)}^3$, we have by Lemma ~\ref{lem:ChebyshevControl}:
    \[\max_{a \in 1, 2, \dots, p}\frac{1}{n}\sum_{i=1}^{n}\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2 \leq 4\norm{\bSig}_{op} \E S_{(i,a)}^3\]
    So that on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap \mathcal{A}_B
    \cap \mathcal{A}_T$, 
    \begin{align*}
    \max_{a \in
    1, 2, \dots,
            p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
            \widehat{\bX}_{ia}\right)^2} &\leq 4\norm{\bSig}_{op} \E S_{(i,a)}^3 C_A \sqrt{\frac{\log{2np}}{n}} 
    \end{align*}
    We are thus ready to conclude the entire term B.  On the event $\mathcal{A}_M \cap \mathcal{A}_O \cap \mathcal{A}_B
    \cap \mathcal{A}_T \cap \mathcal{A}_C$:
    \begin{align*}
    \norm{\frac{1}{n}\left(\widetilde{\bX} -
            \widehat{\bX}\right)^T\left(\widetilde{\bX} -
            \widehat{\bX}\right)\bbe_0}_{\infty} &\leq 4\norm{\bSig}_{op} \E
            S_{(i,a)}^3 C_A C_B R\sqrt{s} \frac{\log{2np}}{n}
    \end{align*}
    The difficult work is done and we are now ready to tackle term C:
    \begin{align*}
    \norm{\frac{1}{n}\left(\widetilde{\bX} -
            \widehat{\bX}\right)^T\left(\widehat{\bX} -
            \bX\right)\bbe_0}_{\infty} &\leq \max_{a \in
    1, 2, \dots,
        p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
        \widehat{\bX}_{ia}\right)^2}
        \cdot R\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left\langle \widehat{\bX}_i -
        \bX_i, \widetilde{\bbe}_0 \right\rangle^2} 
    \end{align*}
    where $\widetilde{\bbe}_0 = \frac{\bbe_0}{\norm{\bbe_0}_2}$.  Notice that
    the vector $\widehat{\bX}_{i} - \bX_i$ is sub-Gaussian with
    parameter $4 \norm{\bSig}_{op}$.  Define then the event $\mathcal{A}_V$ when
    $\frac{1}{n}\sum_{i=1}^{n}\left\langle \widehat{\bX}_i -
        \bX_i, \widetilde{\bbe}_0 \right\rangle^2 \leq 2 \E\left\langle \widehat{\bX}_i -
        \bX_i, \widetilde{\bbe}_0 \right\rangle^2$.  Notice also that:
        \begin{align*}
        \E\left\langle \widehat{\bX}_i -
            \bX_i, \widetilde{\bbe}_0 \right\rangle^2 &\leq \sum_{a,b}
            \left\lvert \widetilde{\bbe}_{0,a} \widetilde{\bbe}_{0,b} \right  \rvert \E \left
            \lvert \hat{\bX}_{ia} - \bX_{ia}\right\rvert^2  \\
            &\leq 4\sum_{a,b} \left\lvert \widetilde{\bbe}_{0,a}
            \widetilde{\bbe}_{0,b} \right \rvert \E
            X_{ia}^2 \\
            &\leq 4\norm{\bSig}_{op} \norm{\widetilde{\bbe}_0}_1^2
        \end{align*}
        where the first inequality is by Cauchy Schwarz and the second by
        Jensen's inequality.  Applying Lemma~\ref{lem:subGaussianSquared} and
        Markov's inequality as we have many times, we obtain:
        \begin{align*}
            \pr\left\{\frac{1}{n}\sum_{i=1}^{n}\left\langle \widehat{\bX}_i -
        \bX_i, \widetilde{\bbe}_0 \right\rangle^2 -  \E\left\langle \widehat{\bX}_i -
            \bX_i, \widetilde{\bbe}_0 \right\rangle^2 \geq t\right\} &\leq
            \text{exp}{-\frac{nt^2}{1024e^2\norm{\bSig}_{op}^2}}
        \end{align*}
        for all $t < 32e\norm{\bSig}_{op}$.  Setting $t = \norm{\bSig}_{op}$
        yields $\pr\left\{\mathcal{A}_V^C\right\} \leq e^{-\frac{n}{1024e^2}}$.
        Thus, we have on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap \mathcal{A}_B
    \cap \mathcal{A}_T \cap \mathcal{A}_V$,
    \begin{align*}
    \norm{\frac{1}{n}\left(\widetilde{\bX} -
            \widehat{\bX}\right)^T\left(\widehat{\bX} -
            \bX\right)\bbe_0}_{\infty} &\leq 8\norm{\bSig}_{op}^{3/2} \E S_{(i,a)}^3
            C_A \sqrt{\frac{s\log{2np}}{n}}
    \end{align*}
    Finally, assume under the assumptions of Theorem~\ref{thm:mainres} and let
    the event $\mathcal{A}_X$ be that
    $\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
    \bX\right)\bbe_0}_{\infty} \leq A
    64\sqrt{2}e\sqrt{c}\norm{\bSig}_{op}\sqrt{1 -
    \alpha}\sqrt{\frac{\log{p}}{n}}$ and notice that
    $\pr\left\{\mathcal{A}_X\right\} \geq 1 - 2p^{2 - A^2}$.  
    Thus, we have (on the events defined above):
    \begin{align*}
    \frac{1}{n}\norm{\widetilde{\bX}^T\left(\widetilde{\bX} -
        \bX\right)\bbe_0}_{\infty} &\leq 9e\norm{\bSig}_{op} C_B
        R\sqrt{\frac{s\log{2np}}{n}} + 4\norm{\bSig}_{op} \E S_{(i,a)}^3 C_A C_B
        R \sqrt{s} \frac{\log{2np}}{n} \\
        &+ 8\norm{\bSig}_{op}^{3/2} \E S_{(i,a)}^3
            C_A \sqrt{\frac{s\log{2np}}{n}} + A
    64\sqrt{2}e\sqrt{c}\norm{\bSig}_{op}\sqrt{1 -
    \alpha}\sqrt{\frac{\log{p}}{n}}  \\
        &\leq C\left(\lambda_{\min}\left(\bSig\right), \norm{\bSig}_{op},
        \alpha, d_{\max}\right) R \sqrt{\frac{s \log{2np}}{n}}
    \end{align*}
    where $C\left(\lambda_{\min}\left(\bSig\right), \norm{\bSig}_{op},
        \alpha, d_{\max}\right)$ is a dimension-independent constant depending
        only on its arguments.
    It remains to
    tackle the quantities $\frac{1}{n}\norm{\widetilde{\bX}\beps}_{\infty}$ as
    well as $\sup_{\bw \in
    S^{p-1}\cap \mathcal{C}}\frac{1}{n}\norm{\widetilde{\bX}\bw}_2^2$. We first work on the former
    term.  We write:
    \begin{align*}
    \norm{\frac{1}{n}\widetilde{\bX}^T\beps}_{\infty} \leq
        \norm{\frac{1}{n}\left(\widetilde{\bX} -
        \widehat{\bX}\right)^T\beps}_{\infty} +
        \norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty}
    \end{align*}
    We notice that the second term was handled under the assumptions of
    Theorem~\ref{thm:mainres}, and we focus on the first term, writing:
    \begin{align*}
    \norm{\frac{1}{n}\left(\widetilde{\bX} -
        \widehat{\bX}\right)^T\beps}_{\infty} &= \max_{a = 1, 2, \dots, p}
        \left\lvert \frac{1}{n}\sum_{i=1}^{n} \left(\widetilde{\bX}_{ia} -
        \widehat{\bX}_{ia}\right)\beps_i \right\rvert \\
        &\leq \max_{a = 1, 2, \dots,
        p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
        \widehat{\bX}_{ia}\right)^2}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\beps_i^2}
    \end{align*}
    Notice that on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap
    \mathcal{A}_B \cap \mathcal{A}_T$, 
    \begin{align*}
    \max_{a = 1, 2, \dots,
        p}\sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\widetilde{\bX}_{ia} -
        \widehat{\bX}_{ia}\right)^2} \leq 4\norm{\bSig}_{op}\E S_{(i,a)}^3 C_A
        \sqrt{\frac{\log{2np}}{n}}
    \end{align*}
    Now define the event $\mathcal{A}_E$ such that $\frac{1}{n}\sum_{i=1}^{n}
    \beps_i^2 \leq 2\sigma^2$ and notice that by
    Lemma~\ref{lem:subGaussianSquared} and Markov's inequality, we have
    $\pr\left\{\mathcal{A}_E^C\right\} \leq
    \text{exp}\left\{-\frac{n}{64e^2\sigma^2}\right\}$.
    Thus, 
    \begin{align*}
        \norm{\frac{1}{n}\widetilde{\bX}^T\beps}_{\infty} &\leq 4\sigma^2\norm{\bSig}_{op}\E S_{(i,a)}^3 C_A
        \sqrt{\frac{\log{2np}}{n}} \\ 
        &= C\left(\sigma, \norm{\bSig}_{op}, \alpha,
        d_{\max}\right)\sqrt{\frac{\log{2np}}{n}}
    \end{align*}
    on the event $\mathcal{A}_M \cap \mathcal{A}_O \cap
    \mathcal{A}_B \cap \mathcal{A}_T \cap \mathcal{A}_E$.  
    Now, we check the restricted eigenvalue condition: $\sup_{\bw \in
    S^{p-1}\cap \mathcal{C}}\frac{1}{n}\norm{\widetilde{\bX}\bw}_2^2$.  Recall
    the decomposition from the proof of Theorem~\ref{thm:ARres}:
    \begin{align*}
    \sup_{\bw \in \mathcal{C} \cap S^{p-1}}\frac{1}{n}\norm{\bX \bw}_2^2 &\geq \sup_{\bw \in \mathcal{C} \cap S^{p-1}} \frac{1}{n}\norm{\hat{\bX}\bw}_2^2
    - \norm{\bw}_1\Biggl(\norm{\left(\tilde{\bX} - \hat{\bX}\right)^T\left(\tilde{\bX} -
    \hat{\bX}\right)\bw}_{\infty} \\
    &+ \norm{\left(\tilde{\bX} -
    \hat{\bX}\right)^T\hat{\bX}\bw}_{\infty} + \norm{\hat{\bX}^T\left(\tilde{\bX} -
    \hat{\bX}\right)\bw}_{\infty} \Biggr) \\
    \end{align*}
    On the events above, and noticing that $\norm{\bw}_1 \leq \sqrt{s}$ by
    Cauchy Schwarz, we see that the negative term is upper bounded by 
    $C\left(\lambda_{\min}\left(\bSig\right), \norm{\bSig}_{op},
        \alpha, d_{\max}\right) s \sqrt{\frac{\log{2np}}{n}}$.  Under the
        assumption $C\left(\lambda_{\min}\left(\bSig\right), \norm{\bSig}_{op},
        \alpha, d_{\max}\right) s \sqrt{\frac{\log{2np}}{n}} \leq
        \frac{\lambda_{\min}\left(\bSig_{\widehat{\bX}}\right)}{4}$, we have the
        restricted eigenvalue condition.
    It remains only to
    check that these events hold with high probability.  We are interested in
    the event:
    \begin{align*}
        \pr\left\{\bigcap_{I = \left\{X, M, O, B, T, V, C,
        S\right\}}\mathcal{A}_I\right\} \geq 1 - \sum_{I = \left\{X, M, O, B, T, V, C,
        S\right\}} \pr\left\{\mathcal{A}_I^C\right\}
    \end{align*}
    We now enumerate each of these probabilities:
    \begin{itemize}
        \item[\bf $\mathcal{A}_O$:] Recall that $\mathcal{A}_O = \left\{\norm{\bW_{S_{(i,b)},
        S_{(i,b)}}}_{op} \leq
            \frac{64e(1-\alpha)\norm{\bSig}_{op}}{\alpha^2}\sqrt{\frac{|S_{(i,b)}| +
            2\log{2np}}{n}} \right\}$.  Notice that by
            Lemma~\ref{lem:operatorMissing} i. and a union bound,
            $\pr\left\{\mathcal{A}_O^C\right\} \leq \frac{1}{2np}$
        \item[\bf $\mathcal{A}_B$:] Recall $\mathcal{A}_B = \left\{|S(i,b)| \leq
\frac{2}{C_B(\alpha, d_{\max})}\log{2np} \quad \forall i \in [n], b \in
[p]\right\}$ and notice that Lemma ~\ref{lem:generatingFunctionBoundary} implies
$\pr\left\{\mathcal{A}_B\right\} \geq 1 - \frac{1}{2np}$
        \item[\bf $\mathcal{A}_M$:] Note that $\mathcal{A}_M$ is the event that
            $\norm{\widetilde{\bSig} - \bSig}_{\ell_1 \rightarrow
        \ell_{\infty}} \leq \frac{64
            e\norm{\bSig}_{op}}{\alpha^2}\sqrt{\frac{\log{p}}{n}}$.  By
            Lemma~\ref{lem:operatorMissing} ii.,
            $\pr\left\{\mathcal{A}_M^C\right\} \leq \frac{1}{p}$.
        \item[\bf $\mathcal{A}_C$:] Recall that $\mathcal{A}_C$ denotes the
            event 
            \begin{align*}
                \frac{1}{n}\sum_{i=1}^{n}\underbrace{\left(\sum_{b=1}^{p}\left\lvert\bbe_{0,b}\right\rvert\sqrt{S_{(i,b)}}\sum_{j
                \in S_{(i,b)}}\left\lvert\bX_{ij}\right\rvert\right)^2}_{C_i} \leq
            \norm{\bSig}_{op}R^2s \left(\E S_{(i,b)}^3 + \sqrt{3 \E
            S_{(i,b)}^6}\right)
            \end{align*}
            Notice that by Chebyshev Inequality $\pr\left\{\sum_{i=1}^{n} C_i - \E C_i \geq t\right\} \leq
                \frac{\text{Var}\left(C_1\right)}{nt^2}$.  Additionally,
            By Lemma ~\ref{lem:ChebyshevControl} setting $t = 3 \E S_{(i,b)}^6
            \norm{\bSig}_{op}^2 R^4s^2$, we have
            $\pr\left\{\mathcal{A}_C^C\right\} \leq \frac{1}{n}$.
        \item[\bf $\mathcal{A}_S$:] Recall that this is the event $\max_{a=1, 2,
            \dots, p}\frac{1}{n}\sum_{i=1}^{n}\bX_{ia}^2 \leq \norm{\bSig}_{op}
            + 16e\norm{\bSig}_{op}\sqrt{\frac{\log{p}}{n}}$.  By the
            calculations earlier in the proof, we note that we have shown
            $\pr\left\{\mathcal{A}_S^C\right\} \leq \frac{1}{p}$.
        \item[\bf $\mathcal{A}_T$:] Recall that denotes the event that:
            \[\max_{a \in 1, 2, \dots, p}\frac{1}{n}\sum_{i=1}^{n}\left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2 \leq
        2\left(A\sqrt{\frac{(\log{c_1 np})^7}{n}} + \E \left(\sqrt{S_{(i,a)}}\sum_{j
        \in S_{(i,a)}} \left\lvert\bX_{ij}\right\rvert\right)^2\right) \]
            and additionally recall that
    $\pr\left\{\mathcal{A}_T\right\} \geq 1 - \text{exp}\left\{\left(1 - c_2
    A^{2/7}\right)\log{c_1 np}\right\}$ where $c_1 = 2 + \frac{4}{1 -
            e^{-C_B(\alpha, d_{\max})/2}}$ and $c_2 = a \left(\frac{a -
    ae^{-C_B(\alpha, d_{\max})/2}}{1024e^2}\right)^{1/7}$ where $A$ is a
            constant such that $A\sqrt{\frac{(\log{c_1 np})^7}{n}} \leq
    \norm{\bSig}_{op} \E S_{(i,a)}^3$.
        \item[\bf $\mathcal{A}_V$:] We have denoted the event $\mathcal{A}_V$
            for when $\frac{1}{n}\sum_{i=1}^{n}\left\langle \widehat{\bX}_i -
        \bX_i, \widetilde{\bbe}_0 \right\rangle^2 \leq 2 \E\left\langle \widehat{\bX}_i -
            \bX_i, \widetilde{\bbe}_0 \right\rangle^2$ and noted that
            $\pr\left\{\mathcal{A}_V^C\right\} \leq e^{-\frac{n}{1024e^2}}$.
        \item[\bf $\mathcal{A}_X$:] Recall $\mathcal{A}_X$ is defined as $\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
    \bX\right)\bbe_0}_{\infty} \leq A
    64\sqrt{2}e\sqrt{c}\norm{\bSig}_{op}\sqrt{1 -
    \alpha}\sqrt{\frac{\log{p}}{n}}$ and notice that
    $\pr\left\{\mathcal{A}_X\right\} \geq 1 - 2p^{2 - A^2}$
        \item[\bf $\mathcal{A}_E$:] This is the event that
            $\frac{1}{n}\sum_{i=1}^{n}\beps_i^2 \leq 2\sigma^2$ and notice that
            we have shown $\pr\left\{\mathcal{A}_E^C\right\} \leq
            e^{-\frac{n}{64e^2\sigma^2}}$.
    \end{itemize}
    
\end{proofof}


==> ProofsConditionalExpectation.tex <==
The proofs of our results follows a standard outline for $\ell_1$--regularized objective
functions as can be found in e.g., Bickel et al.~\cite{bickel2009simultaneous}.
We provide the proof of this generalization in Appendix ~\ref{sec:GeneralLasso}.
\begin{proposition} 
\label{prop:GeneralLasso}    
Given a design matrix $\widetilde{\bX} \in \mathbb{R}^{n \times p}$ and $\lambda>0$, consider the solution to the convex program
\begin{align*}
\widetilde{\bbe} \in \argmin_{\bbe \in \mathbb{R}^p} \left\{\frac{1}{2n}\norm{\by -
\widetilde{\bX}\bbe}_2^2 + \lambda \norm{\bbe}_1\right\}.
\end{align*}
Further, assume
\begin{align*}
&\norm{\frac{1}{n}\widetilde{\bX}^T\left(\widetilde{\bX} -\bX\right)\bbe_0}_{\infty} \leq \frac{\lambda}{4}, 
\hspace{.5cm}
\norm{\frac{1}{n}\widetilde{\bX}^T\beps}_{\infty} \leq \frac{\lambda}{4},\\
&\text{and}~~~~
\sup_{\bw \in \mathcal{C} \cap \mathcal{S}^{p-1}}\frac{1}{n}\norm{\widetilde{\bX}\bw}_2^2 \geq \kappa,
\end{align*} 
where $\mathcal{C}$ is the cone $\mathcal{C} = \left\{\bw \in \mathbb{R}^p: \norm{\bw_{S^c}}_1 \leq
    3\norm{\bw_S}_1\right\}$.
Then $\norm{\widetilde{\bbe} - \bbe_0}_2 \leq \frac{12\lambda\sqrt{s}}{\kappa}$.
\end{proposition}
\noindent We are now prepared to prove our main results.
\subsection{Proof of Theorem ~\ref{thm:mainres} and Corollary
~\ref{cor:IdentityCovariance}}
\vspace{.2cm}
\noindent\begin{proofof}{Theorem~\ref{thm:mainres}}
We show that the assumptions of Proposition~\ref{prop:GeneralLasso} are satisfied with high probability by setting 
\[\widehat{\lambda} = 4A\sigma_X\left(\psi_1(\sigma) + \psi_2(\sigma_X,
    \alpha)R\right)\sqrt{\frac{\log{p}}{n}}\]
and  $\kappa =\frac{
\lambda_{\text{min}}\left(\Sigma_{\widehat{\bX}}\right)}{2}$.  The theorem then follows
directly as a consequence.  Before tackling each of the
    assumptions of Proposition~\ref{prop:GeneralLasso}, we state and prove the
    following fact that we will use repeatedly.
\begin{fact}
\label{fact:subGaussianConditionalExpectation}
$\widehat{\bX}_i = \E\left\{\bX \mid \bX_{S}\right\}$ is sub-Gaussian with
    parameter $\sigma_X^2$.
\end{fact}
\noindent\begin{proofof}{Fact~\ref{fact:subGaussianConditionalExpectation}}
   \begin{align*}
\label{eq:condExpSubGaussian}
\E\left\{e^{\lambda\inp{\bu}{\widehat{\bX}_i}}\right\} \leq
\E\left\{\E\left\{e^{\lambda\inp{\bu}{\bX_i}}\mid \bX_S\right\}\right\} =
\E\left\{e^{\lambda\inp{\bu}{\bX_i}}\right\} \leq e^{\lambda^2\sigma_X^2}
\end{align*} 
\end{proofof}
\noindent 
    
\noindent We now tackle each of the
assumptions:
\begin{enumerate}[align=left]
\item[I.] We would like to show that
$\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty} \leq
\frac{\widehat{\lambda}}{4}$.  We write:
\begin{align*}
\norm{ \frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
                \bX\right)\bbe_0 }_{\infty} &= \norm{\bbe_0}_2 \max_{a=1, 2, \dots, p} \left\lvert
                \frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\widetilde{\bbe}_{0,b} \right \rvert
\end{align*}
        where $\widetilde{\bbe_0} = \frac{\bbe_0}{\norm{\bbe_0}}$.  We will
        require the following lemma, whose proof we defer to
        Appendix~\ref{sec:appendixConditionalExpectation}:
            \begin{lemma}
            \label{lem:subexpMCAR}
            Let $c_X = 16e\sigma_X^2$ and $\lambda_c, c$ such that
                $e^{\frac{1}{2}c_X^2
                \lambda_c^2} + \lambda_c^2c_X^2e^{\frac{1}{2}c_X^2
                \lambda_c^2} \leq c$.  Then $\forall \lambda \leq \lambda_c
                \wedge \frac{1}{16e\sigma_X^2}$:
                \begin{align*}
                    \E\text{exp}\left\{\lambda\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\widetilde{\bbe}_{0,b}\right\} \leq
                    e^{\frac{1}{2}c(1 -
                \alpha)c_X^2\lambda^2}
                \end{align*} 
            \end{lemma}
            \begin{remark}
            For instance, taking $c=2$, $\lambda_c = \frac{1}{16\sqrt{2}e
                \sigma_X^2}$ satisfies the conditions.
            \end{remark}
            Thus, a union bound implies:
            \begin{align*}
                \pr\left\{\max_{a=1, 2, \dots, p} \left\lvert
                \frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\widetilde{\bbe}_{0,b} \right \rvert \geq t\right\} &\leq 2p \pr
                    \left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\left\langle
                    \bX_i - \widehat{\bX}_i, \widetilde{\bbe}\right\rangle\geq t\right\}
            \end{align*} 
            Suppose that $\frac{t}{c(1 - \alpha)c_X^2} \leq \lambda_c \wedge
            \frac{1}{16e\sigma_X^2}$, then Lemma~\ref{lem:subexpMCAR} implies:
            \begin{align*}
                2p\pr
                    \left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\left\langle
                    \bX_i - \widehat{\bX}_i, \widetilde{\bbe}\right\rangle\geq
                    t\right\} 
                    &\leq \text{exp}\left\{\log{2p} -\frac{t^2n}{2c(1 -
                    \alpha)c_X^2}\right\}
            \end{align*}
    \item[II.] We show
    $\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty} \leq
        \frac{\widehat{\lambda}}{4}$.  The proof follows directly from the
        following well-known lemma regarding the product of sub-Gaussian random
        variables, whose proof we give in
        Appendix~\ref{sec:appendixConditionalExpectation}
        \begin{lemma}
\label{lem:productsubGaussian}
Let $X$ be $\sigma_X^2$ sub-Gaussian and $Y$ be $\sigma_Y^2$ sub-Gaussian.
Assume also that $X, Y, XY$ are all $0$-mean.
Then, $\forall \lambda \leq \frac{1}{8e\sigma_X \sigma_Y}$:
\[\E e^{\lambda XY} \leq e^{\lambda^2 32e^2 \sigma_X^2 \sigma_Y^2}\]
\end{lemma}

Notice that we may re-write $\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty} =
\max_{a \in [p]}\left\lvert
\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i\right\rvert$.  We see that by
the union bound:
\begin{align*}
    \pr\left\{\max_{a \in [p]}\left\lvert
\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i\right\rvert \geq t\right\}
    \leq 2p \pr\left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i \geq t\right\}
\end{align*}
Supposing that $t \leq 8e\sigma_X \sigma$, Lemma~\ref{lem:productsubGaussian}
implies:
\begin{align*}
2p \pr\left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i \geq t\right\}
    \leq \text{exp}\left\{\log{2p} - \frac{t^2n}{64e^2\sigma_X^2\sigma^2}\right\}
\end{align*}
Noting that for $p \geq 2$, $p^2 \geq 2p$, and taking $t =
A\sqrt{\frac{\log{p}}{n}}\left(8e\sigma_X\sigma + 16\sqrt{2}e\sigma_X^2
\sqrt{c(1 - \alpha)}\right)$, we have:
\begin{align*}
    \pr\left\{\left\{\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty} \leq
    \frac{\widehat{\lambda}}{4}\right\} \cap \left\{\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty} \leq
        \frac{\widehat{\lambda}}{4}\right\}\right\} \geq 1 - 2p^{2 - A^2}
\end{align*}
    
\item[III.]  Finally, we aim to show that $\sup_{\bw \in \mathcal{C} \cap
\mathcal{S}^{p-1}}\frac{1}{n}\norm{\tilde{\bX}\bw}_2^2 \geq
\frac{\lambda_{\text{min}}\left(\Sigma_{\widehat{\bX}}\right)}{2}$.  We will
require the following proposition:
\begin{proposition} 
    \label{prop:RE_Condition}
Let $\bX$ be a matrix with i.i.d. rows, each of which is sub-Gaussian with
    parameter $\sigma_X^2$ and has covariance matrix $\Sigma_{\bX}$.
    Then  $\bX$ satisfies a
                    restricted eigenvalue condition:
    \begin{align*}
        \sup_{\bw \in \mathcal{C} \cap S^{p-1}}\frac{1}{n}\norm{\bX \bw}_2^2
        \geq \frac{\lambda_{\text{min}}\left(\Sigma_X\right)}{2}
    \end{align*}
    with probability at least 
    \begin{align*}
        1 -
                2\text{exp}\left\{-c n \left(\min\left(\frac{t^2}{\sigma_X^4},
                \frac{t}{\sigma_X^2}\right) + \frac{s \log{p}}{n}\right)\right\}
    \end{align*}
    where $\mathcal{C}$ is the cone $\mathcal{C} = \left\{\bw \in \mathbb{R}^p: \norm{\hat{\bw}_{S^c}}_1 \leq
    3\norm{\hat{\bw}_S}_1\right\}$.
\end{proposition}
The result follows immediately from Proposition ~\ref{prop:RE_Condition} and
Fact~\ref{fact:subGaussianConditionalExpectation}. 
\end{enumerate}
\end{proofof}

\noindent \begin{proofof}{Corollary~\ref{cor:IdentityCovariance}}
This proof is almost identitical to the proof of the previous theorem.  It is
    possible, however, to tighten the analysis of
    $\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
    \bX\right)\bbe_0}_{\infty}$ and
    $\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty}$. As before, we write
    \begin{align*}
\norm{ \frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
                \bX\right)\bbe_0 }_{\infty} &= \norm{\bbe_0}_2 \max_{a=1, 2, \dots, p} \left\lvert
                \frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\widetilde{\bbe}_{0,b} \right \rvert
\end{align*}
    Now we have for $\lambda \leq \left(\frac{1}{\sqrt{1 - \alpha} \sqrt{ce}
    16e}\right) \wedge \lambda_c \wedge \frac{1}{16e}$: 
    \begin{align*}
        \E \text{exp}\left\{\lambda \widehat{\bX}_{ia}\left\langle \bX_i -
        \widehat{\bX}_i, \widetilde{\bbe_0}\right \rangle\right\} &= (1 -
        \alpha) + \alpha \E \text{exp}\left\{\lambda \bX_{ia}\sum_{b \neq
        a}\left(\bX_{ib} -
        \widehat{\bX}_{ib}\right)\widetilde{\bbe}_{0,b}\right\}\\
        &\leq (1 - \alpha) +
        \alpha\text{exp}\left\{\frac{1}{2}c(1-\alpha)c_X^2\lambda^2\right\} \\
        &= 1 +
        \alpha\sum_{k=1}^{\infty}\frac{\left(\frac{1}{2}c(1-\alpha)c_X^2\lambda^2\right)^k}{k!}\\
        &\leq 1 +
        \alpha\sum_{k=1}^{\infty}\frac{\left(\frac{1}{2}c(1-\alpha)c_X^2\lambda^2\right)^k
        k^k}{k!} \\
        &\leq 1 + \alpha
        \sum_{k=1}^{\infty}\left(\frac{1}{2}ce(1-\alpha)c_X^2\lambda^2\right)^k\\
        &\leq \text{exp}\left\{ce\alpha(1 - \alpha)c_X^2\lambda^2\right\}
    \end{align*}
    where the first inequality is by conditioning on whether the $ia$th entry is
    missing or not and the first inequality is by Lemma~\ref{lem:subexpMCAR}.
    Suppose that $\frac{t}{2ce\alpha(1 - \alpha)c_X^2} \leq \lambda_c \wedge
            \frac{1}{16e} \wedge \frac{1}{\sqrt{1 - \alpha} \sqrt{ce}
    16e}$, then the above implies:
            \begin{align*}
                2p\pr
                    \left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\left\langle
                    \bX_i - \widehat{\bX}_i, \widetilde{\bbe}\right\rangle\geq
                    t\right\} 
                    &\leq \text{exp}\left\{\log{2p} -\frac{t^2n}{4ce\alpha(1 -
                    \alpha)c_X^2}\right\}
            \end{align*}
    Proceeding similarly, but invoking Lemma~\ref{lem:productsubGaussian} in
    place of Lemma~\ref{lem:subexpMCAR}, we see that for $\lambda <
    \frac{1}{8e^{3/2}\sigma}$,
    $\E\left\{e^{\lambda\widehat{\bX}_{ia}\beps_i}\right\} \leq
    \text{exp}\left\{\lambda^2 64e^3\sigma^2\alpha\right\}$, which implies for
    $t < 16e^{3/2}\sigma\alpha$:
    \begin{align*}
2p \pr\left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i \geq t\right\}
    \leq \text{exp}\left\{\log{2p} - \frac{t^2n}{256e^3\sigma^2\alpha}\right\}
\end{align*}
Noting that for $p \geq 2$, $p^2 \geq 2p$, and taking $t =
    A\sqrt{\frac{\log{p}}{n}}\left(16e^{3/2}\sigma + 32e^{3/2}
\sqrt{c\alpha(1 - \alpha)}\right)$, we have:
\begin{align*}
    \pr\left\{\left\{\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty} \leq
    \frac{\widehat{\lambda}}{4}\right\} \cap \left\{\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty} \leq
        \frac{\widehat{\lambda}}{4}\right\}\right\} \geq 1 - 2p^{2 - A^2}
\end{align*}
\end{proofof}

\subsection{Proof of Theorem~\ref{thm:mnar}}
\label{sec:ProofMNAR}
The proof of this theorem largely follows the same recipe as for the case with
MCAR data, however, we allow ourselves to use coarser bounds to relax the
dependence on $\alpha$.

\noindent \begin{proofof}{Theorem~\ref{thm:mnar}}
The proof again follows the strategy outlined by
    Proposition~\ref{prop:GeneralLasso}.  The restricted eigenvalue condition
    and the analysis of the term
    $\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty}$ are identitical to those
    in Theorem~\ref{thm:mainres}, so we focus only on the term $\norm{ \frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
                \bX\right)\bbe_0 }_{\infty}$.
 We first re-write 
            \begin{align*}\norm{ \frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} -
                \bX\right)\bbe_0 }_{\infty} &= \max_{i=1, 2, \dots, p} \left\lvert
            \left\langle \be_i, \frac{1}{n}\widehat{\bX}\left(\bX - \widehat{\bX
            }\right)\bbe_0\right\rangle\right\rvert \\
                &= \frac{\norm{\bbe_0}_2}{n} \max_{i=1, 2, \dots, p} \left\lvert
                \left\langle \widehat{\bX}\be_i, \left(\bX - \widehat{\bX
                }\right)\widetilde{\bbe_0}\right\rangle\right\rvert\\
                &= \frac{\norm{\bbe_0}_2}{2} \max_{i=1, 2, \dots, p}\Biggl
                \lvert \frac{1}{n}\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\widetilde{\bbe_0}}_2^2 - \E\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\widetilde{\bbe_0}}_2^2 \\
                & - \left(\frac{1}{n}\norm{\widehat{\bX}\be_i}_2^2 -
                \E\norm{\widehat{\bX}\be_i}_2^2\right) - \left(\frac{1}{n}\norm{\left(\bX -
                \widehat{\bX}\right)\widetilde{\bbe_0}}_2^2 - \E\norm{\left(\bX -
                \widehat{\bX}\right)\widetilde{\bbe_0}}_2^2\right)\Biggr\rvert
            \end{align*}
            where $\widetilde{\bbe_0} = \frac{\bbe_0}{\norm{\bbe_0}}$.  The last
            equality follows from noticing that for any two fixed vectors $\bx,
            \by$, we have $\langle \bx, \by \rangle = \frac{1}{2}\left(\norm{\bx +
            \by}_2^2 - \norm{\bx}_2^2 - \norm{\by}_2^2\right)$ as well as that $\E\left\langle \widehat{\bX}\be_i, \left(\bX - \widehat{\bX
                }\right)\widetilde{\bbe_0}\right\rangle = 0$ by the orthogonality
                property of the conditional expectation.
Our remaining strategy is to upper bound
            \begin{align*}
                &\pr\Biggl\{\Biggl \lvert \frac{1}{n}\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2  \nonumber\\
                  &- \left(\frac{1}{n}\norm{\widehat{\bX}\be_i}_2^2 -
                \E\norm{\widehat{\bX}\be_i}_2^2\right) - \left(\frac{1}{n}\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2\right)\Biggr\rvert
                \geq t \Biggr\} \nonumber\\
                &\leq \pr\left\{\left\lvert\frac{1}{n}\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 \right\rvert \geq
                \frac{t}{3}\right\}
                \label{eq:union_bound_versh}\\
                & + \pr\left\{\left\lvert \left(\frac{1}{n}\norm{\widehat{\bX}\be_i}_2^2 -
                \E\norm{\widehat{\bX}\be_i}_2^2\right) \right\rvert \geq \frac{t}{3}\right\} +
                \pr\left\{\left\lvert \left(\frac{1}{n}\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2\right)\right\rvert \geq
                \frac{t}{3}\right\}. %\nonumber
            \end{align*}
            Noting that the sum of sub-Gaussian random variables is
            sub-Gaussian, we obtain the following bounds on each of the terms:
            \begin{align*}
                \pr\left\{\left\lvert\frac{1}{n}\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\widehat{\bX}\be_i + \left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 \right\rvert \geq
                \frac{t}{3}\right\} &\leq \text{exp}\left\{-\frac{nt^2}{9 \cdot
                (72e\sigma_X^2)^2}\right\} \\
                \pr\left\{\left\lvert \left(\frac{1}{n}\norm{\widehat{\bX}\be_i}_2^2 -
                \E\norm{\widehat{\bX}\be_i}_2^2\right) \right\rvert \geq
                \frac{t}{3}\right\} &\leq \text{exp}\left\{-\frac{nt^2}{9 \cdot
                (8e\sigma_X^2)^2}\right\} \\
                \pr\left\{\left\lvert \left(\frac{1}{n}\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2 - \E\norm{\left(\bX -
                \widehat{\bX}\right)\tilde{\bbe_0}}_2^2\right)\right\rvert \geq
                \frac{t}{3}\right\} &\leq \text{exp}\left\{-\frac{nt^2}{9 \cdot
                (32e\sigma_X^2)^2}\right\} 
            \end{align*}
            where all three inequalities hold if $t < 24e\sigma_X^2$.  Combining
            these concentration inequalities, with the previously derived
            concentration for $t < 8e\sigma_X \sigma$
            \begin{align*}
 \pr\left\{\frac{1}{n}\sum_{i=1}^{n}\widehat{\bX}_{ia}\beps_i \geq t\right\}
    \leq \text{exp}\left\{- \frac{t^2n}{64e^2\sigma_X^2\sigma^2}\right\}
\end{align*}
and taking a union bound, we see that taking $t = 8e \cdot A \cdot
\sigma_X\left(\sigma + 27 \sigma_X\right)\sqrt{\frac{\log{p}}{n}}$ implies
\begin{align*}
    \pr\left\{\left\{\norm{\frac{1}{n}\widehat{\bX}^T\left(\widehat{\bX} - \bX\right)\bbe_0}_{\infty} \leq
    \frac{\widehat{\lambda}}{4}\right\} \cap \left\{\norm{\frac{1}{n}\widehat{\bX}^T\beps}_{\infty} \leq
        \frac{\widehat{\lambda}}{4}\right\}\right\} \geq 1 - 2p^{2 - A^2}
\end{align*}
the proof of the restricted eigenvalue condition is identitical to
Theorem~\ref{thm:mainres} and we are done.
\end{proofof}


==> SubExpMCAR.tex <==
\subsection{Proof of Lemma~\ref{lem:productsubGaussian}}
Recall the statement: 
\begin{customlemma}{A.4}
Let $X$ be $\sigma_X^2$ sub-Gaussian and $Y$ be $\sigma_Y^2$ sub-Gaussian.
Assume also that $X, Y, XY$ are all $0$-mean.
Then, $\forall \lambda \leq \frac{1}{8e\sigma_X \sigma_Y}$:
\[\E e^{\lambda XY} \leq e^{\lambda^2 32e^2 \sigma_X^2 \sigma_Y^2}\]
\end{customlemma}
\noindent\begin{proofof}{Lemma~\ref{lem:productsubGaussian}}
Taylor expanding $e^{\lambda XY}$ gives: 
\begin{align*}
\E e^{\lambda XY} \leq 1 +
\sum_{k=2}^{\infty} \frac{\lambda^{k}\E |XY|^{k}}{k!} \leq 1 +
\sum_{k=2}^{\infty} \frac{\lambda^{k} \sqrt{\E |X|^{2k} \E |Y|^{2k}}}{k!}
\end{align*}
where the first inequality follows since $\E XY = 0$ and $XY \leq |XY|$ and the
second inequality follows by Cauchy-Schwarz.  Now,
\begin{align}
\label{eq:2k_moment}
\E |X|^{2k} = \int_{0}^{\infty} 2k t^{2k-1} \Pr\left\{|X| \geq t\right\} dt = 2k
(2\sigma_X^2)^k \Gamma(k)
\end{align}
where $\Gamma(k) = \int_{0}^{\infty} t^{k-1}e^{-t}dt$.  Stirling's inequality
gives $\Gamma(k) \leq k^{k}$ and noting that $2k \leq 2^{k}$ for $k \geq 2$
implies $\E |X|^{2k} \leq (4\sigma_X^2)^{k} k^{k}$.  Proceeding similarly for
$\E |Y|^{2k}$ yields 
\[1 +
\sum_{k=2}^{\infty} \frac{\lambda^{k} \sqrt{\E |X|^{2k} \E |Y|^{2k}}}{k!} \leq 1
+ \sum_{k=2}^{\infty} \frac{\lambda^k (4\sigma_X \sigma_Y)^k k^k}{k!} \leq 1 +
\sum_{k=2}^{\infty}(4\lambda e \sigma_X \sigma_Y)^k = 1 + \frac{(4\lambda e
\sigma_X \sigma_Y)^{k}}{1 - 4\lambda e \sigma_X \sigma_Y}\]
where the third inequality used the fact that $k! \geq \frac{k^k}{e^k}$ and the
last equality invoked the sum of a geometric series.  Finally, noting that
$\lambda \leq \frac{1}{8e\sigma_X \sigma_Y}$, we can upper bound 
\[1 + \frac{(4\lambda e
\sigma_X \sigma_Y)^{k}}{1 - 4\lambda e \sigma_X \sigma_Y} \leq 1 +
32e^2\sigma_X^2\sigma_Y^2 \leq e^{\lambda^2 32 e^2 \sigma_X^2 \sigma_Y^2}\]
\end{proofof}

\noindent We will repeatedly make use of the following related lemma whose proof
is nearly identical.
\begin{lemma}
\label{lem:subGaussianSquared}
    Let $X$ be $\sigma_X^2$ sub-Gaussian.  Then, $\forall \lambda \leq
    \frac{1}{8e\sigma_X^2}$:
    \[\E e^{\lambda \left(X^2 - \E X^2\right)} \leq e^{\lambda^2
    32e^2\sigma_X^4}\]
\end{lemma}
\noindent \begin{proofof}{Lemma ~\ref{lem:subGaussianSquared}}
As before, we begin by Taylor expanding $e^{\lambda XY}$ gives: 
\begin{align*}
\E e^{\lambda \left(X^2 - \E X^2\right)} \leq 1 +
\sum_{k=2}^{\infty} \frac{\lambda^{k}\E \left\lvert X^2 - \E X^2\right\rvert^{k}}{k!} \leq 1 +
    \sum_{k=2}^{\infty} \frac{\left(2\lambda\right)^{k} \E |X|^{2k}}{k!}
\end{align*}
    where the last inequality follows by writing $X^2 - \E X^2 = X^2 - \E_{X_1}
    X_1^2$ where $X_1$ is an i.i.d. copy of $X$ and using Jensen's inequality.  The remainder of the proof
    follows exactly as that of Lemma~\ref{lem:productsubGaussian}.
\end{proofof}



\subsection{Proof of Lemma~\ref{lem:subexpMCAR}}
\label{sec:AppendixSubExpMCAR}
We re-state the lemma for convenience:
\begin{customlemma}{A.3}
               Let $c_X = 16e\sigma_X^2$ and $\lambda_c, c$ such that
                $e^{\frac{1}{2}c_X^2
                \lambda_c^2} + \lambda_c^2c_X^2e^{\frac{1}{2}c_X^2
                \lambda_c^2} \leq c$.  Then $\forall \lambda \leq \lambda_c
                \wedge \frac{1}{16e\sigma_X^2}$:
                \begin{align*}
                    \E\text{exp}\left\{\lambda\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\tilde{\bbe}_{0,b}\right\} \leq
                e^{\frac{1}{2}c(1 -
                \alpha)c_X^2\lambda^2}
                \end{align*}  
\end{customlemma}
\noindent\begin{proofof}{Lemma~\ref{lem:subexpMCAR}}
Notice that (here we refer to $S^c$ as $[p] \ S$ for a given set $S$):
            \begin{align*}
            \E\text{exp}\left\{\lambda\widehat{\bX}_{ia}\sum_{b=1}^{p}\left(\bX_{ib} -
                \widehat{\bX}_{ib}\right)\tilde{\bbe}_{0,b}\right\} &= \sum_{S
                \subseteq [p]}\alpha^{\lvert S\rvert}(1 - \alpha)^{p - \lvert S
                \rvert} \E\text{exp}\left\{\lambda\widehat{\bX}_{ia}\left\langle
                \widehat{\bX}_{i,S^c} -
                \bX_{i, S^c}, \tilde{\bbe}_{0,S^c} \right \rangle\right\} \\
                &\leq \sum_{S \subseteq [p]} \alpha^{\lvert S\rvert}(1 -
                \alpha)^{p - \lvert S
                \rvert} e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0, S^c}}_2^2}
                \\ 
                &= \E_S \text{exp}\left\{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                S^c}}_2^2\right\}
            \end{align*}
            where we have used Lemma~\ref{lem:productsubGaussian} and the
            assumption $\lambda \leq \lambda_c
                \wedge \frac{1}{16e\sigma_X^2}$.  Now, define $\phi(\lambda) \equiv \log \E_S
            \text{exp}\left\{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                S^c}}_2^2\right\}$.  Suppose that $\phi(0) = \phi^{'}(0) = 0$
                and for $\lambda \in [0, \lambda_c]$,
                $\phi^{''}(\lambda) \leq c(1 - \alpha)c_X^2$.  Then, we
                have:
                \[\phi(\lambda) = \int_{0}^{\lambda}
                \int_{0}^{t_1}\phi^{''}(t_2)d t_2 d t_1 \leq \frac{\lambda^2 c(1
                - \alpha) c_X^2}{2}\]
                and the result follows immediately.  We now verify the two
                conditions.  By dominated convergence, $\phi^{'}(\lambda) =
                \frac{\lambda c_X^2 \E\norm{\tilde{\bbe}_{0,
                S^c}}_2^2\text{exp}\left\{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                S^c}}_2^2\right\}}{\E_S
            \text{exp}\left\{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                S^c}}_2^2\right\}}$ and thus $\phi(0) = \phi^{'}(0) = 0$.  We
                use dominated convergence once more to calculate
                $\phi^{''}(\lambda)$:
                \begin{align*}
                    \phi^{''}(\lambda) &= c_X^2\frac{\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)}{\E_S\left(e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)} + \lambda^2c_X^4\frac{\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^4e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)}{\E_S\left(e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)} \\
                    &- \lambda^2c_X^4\frac{\left[\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2e^{\frac{1}{2}\lambda^2 c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)\right]^2}{\left[\E_S\left(e^{\frac{1}{2}\lambda^2
                    c_X^2 \norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}\right)\right]^2} \\
                    &= c_X^2\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2 z_S\right) + \lambda^2
                    c_X^4\left(\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^4z_S\right) - \left[\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2z_S\right)\right]^2\right) \\
                    &\leq c_X^2\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2 z_S\right) + \lambda^2
                    c_X^4\left(\E_S\left(\norm{\tilde{\bbe}_{0,
                    S^c}}_2^4z_S\right)\right)
                \end{align*}
                where $z_S = \frac{e^{\frac{1}{2}\lambda^2c_X^2\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}}{\E_Se^{\frac{1}{2}\lambda^2c_X^2\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2}}$.  Notice that
                    $e^{-\frac{1}{2}c_X^2\lambda_c^2} \leq z_S \leq
                    e^{\frac{1}{2}c_X^2\lambda_c^2}$.  Additionally, notice
                    that $\E_S\norm{\tilde{\bbe}_{0,
                    S^c}}_2^2 = 1 - \alpha$ and $\E_S \norm{\tilde{\bbe}_{0,
                    S^c}}_2^4 \leq 1 - \alpha$ (since $\tilde{\bbe}_0$ is a unit
                    norm vector).  We thus see that:
                    \begin{align*}
                        \frac{\phi^{''}(\lambda)}{c_X^2(1 - \alpha)} \leq
                        e^{\frac{1}{2}c_X^2 \lambda_c^2} + \lambda_c^2
                        c_X^2 e^{\frac{1}{2}c_X^2\lambda_c^2} \leq c
                    \end{align*}
                    And we are done.
\end{proofof}

